A three-dimensional model of skeletal muscle tissues

Skeletal muscles are living tissues that can undergo large deformations in short periods of time and that can be activated to produce force. In this paper we use the principles of continuum mechanics to propose a dynamic, fully non-linear, and three-dimensional model to describe the deformation of these tissues. We model muscles as a fibre-reinforced composite and transversely isotropic material. We introduce a flexible computational framework to approximate the deformations of skeletal muscle to provide new insights into the underlying mechanics of these tissues. The model parameters and mechanical properties are obtained through experimental data and can be specified locally. A semi-implicit in time, conforming finite element in space scheme is used to approximate the solutions to the governing nonlinear dynamic model. We provide a series of numerical experiments demonstrating the application of this framework to relevant problems in biomechanics, and also discuss questions around model validation.

==> Manuscript/FromPhDThesis.tex <==
% include path to images for this paper
\graphicspath{{../images/}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{section:3dmuscleintro}
Skeletal muscles are highly complex tissues which play a crucial structural and mechanical role in living beings. A full understanding of the mechanical role of muscle architecture and tissue properties remains an open and challenging scientific problem. Unlike nonliving materials, muscles can be deformed both {\it actively} or {\it passively}. Active deformations are experienced when internal chemical processes and
changes in the shape of proteins are triggered by neuronal signals (see, e.g. \cite{ref:oomens2009,ref:wakeling2020}). Passive deformations describe the mechanical response of the muscle tissue in the presence of external forces \cite{ref:hill1938}.

Muscles can be described as nonlinear elastic materials. The modelling approach in this study is focused on a macroscopic description of muscle and considers muscle {\it fibres} as the smallest unit. These fibres are long and cylindrical cells composed of {\it sarcomeres} arranged in parallel; the sarcomere is the functional unit of muscle fibres. Thousands of these fibres are attached next to each other with {\it connective tissue} between them. The connective tissue in muscles includes the epimysium, perimysium, and endomysium (see \autoref{fig:3dmuscleskeletalmuscle}). Tendon and aponeurosis play an important role in the performance and physiology of muscles. These tissues are composed of collagen fibres, each with its own matrix of {\it bulk} tissue. In tendons, the collagen fibres are arranged in parallel, running from the bone to the muscle. The aponeuroses are thin sheets of tendon-like tissue where the collagen fibres are distributed in a more random fashion.

Muscles possess an intricate internal structure. Muscle fibres render the overall tissue transversely isotropic: its properties are different along the direction of fibres compared to the transverse directions \cite{ref:oomens2009,ref:zatsiorsky2012}. Muscle fibres can be activated, and
they contribute to the transverse elastic properties of an entire muscle. Therefore, a combination of the different distributions of
the muscle fibres and their elastic properties can play a fundamental role in the performance of the muscle as a whole.
Since the overall unit exhibits nonlinear, transversely isotropic behaviour leading to large deformations, we employ
a strain energy formulation, including both volumetric and isochoric contributions. The latter includes
contributions due to the active and passive properties of the muscle, and allows for spatial and structural variations
within the muscle as well as changes to fibre orientations.

It is necessary to investigate the physiological properties of skeletal muscles to be able to understand the function of muscle and to answer questions regarding impairments arising from disease, injury, and disuse (see, e.g. \cite{ref:wakeling2020}). Most of our current understanding of muscle mechanics comes from measurements in sarcomeres, single fibres, small muscles (such as rat muscle), and in silica experiments of 1D nonlinear models. The latter are based on the Hill-type muscle model, introduced by A. V. Hill in \cite{ref:hill1938}. Such models assume that muscles behave as one dimensional nonlinear damped spring systems, and that both mass and inertial effects are negligible. Such models perform well when validated against experimental data of maximal contractions at constant muscle velocity, as well as during isometric contractions (see, e.g. \cite{ref:ross2018-2}, and references therein). An isometric contraction of muscle is considered as an elastic deformation of the tissues in which the ends of the muscle (both attached to bones) are fully clamped. In addition, 1D muscle models do not consider any three dimensional effects of muscle contractions: these have recently proven to be of great importance in terms of the use of the energy in the muscle and its force production, even in the steady-state regime \cite{ref:wakeling2020,ref:ryan2020}.

\sebacomments{Add literature on modelling of muscle (3D, isometric and dynamic).}

In this paper we propose a fully three dimensional and nonlinear system of equations to describe the dynamics of muscle deformation. This models assumes that the mass of the muscle is conserved, and that the tissues behave as nearly incompressible, anisotropic fibre-reinforced materials. Our current model allows us to include and specify the properties of muscle, aponeurosis, tendon, and fat. Each of these possess different mechanical and physiological properties. Muscle fibres and collagen fibres in both the aponeurosis and tendon are described mathematically as one dimensional curves embedded in the three dimensional space. Each fibre is defined as a mapping of tangential unit vectors, referred to as {\it orientation vectors}. The space between the fibres is filled with the {\it base material}; this material includes a combination of intra- and extra-cellular components of muscle, including connective tissue, water, blood, and other materials.

We also introduce a numerical framework to allow the implementation of different experimental setups. Both isometric and dynamic contractions of muscles can be simulated within this framework. in silica experiments have been performed with the use of our framework for isometric contractions to study the energetics of muscle contractions \cite{ref:wakeling2020}, and of compression loads on muscles \cite{ref:ryan2020}. The framework has been used to simulate cyclic contraction \cite{ref:ross2018-2,ref:ross2020} of muscle which mimic the deformations that muscle undergoes during, for example, biking or running. With this framework we are able to specify different mechanical properties of various tissues (muscle, aponeurosis, tendon, fat, and base material), localized fibre orientation vectors, regionalized activation of muscle fibres, as well as import custom-made meshes.

The system of nonlinear equations governing the deformation of skeletal muscle is discretized with a semi-implicit scheme in time and a finite element method in space. We employ the formulation introduced in \cite{ref:simo1985} to approximate the displacement, internal pressure, and dilation of the tissues. A CFL condition links the time step size and the mesh size of the time stepping and finite element discretization, respectively, to ensure the stability of the computations. Our framework is based on the implementation of neo-Hookean materials given in \cite{ref:pelteret2012}. The implementation of the method was done within the finite element library deal.II, version 8.5.1 \cite{ref:davydov2017}.

The rest of this paper is organized as follows. In \autoref{section:3dmusclephysiologyhill} we briefly discuss the physiology of skeletal muscles and give a brief overview of the Hill-type muscle model. In \autoref{section:3dmusclemechanics} we provide an overview of nonlinear elasticity and introduce the system of equations that describe the large deformation of muscles. 
In \autoref{section:3dmusclemethods} we develop the discretization of the continuous problem. Finally, some results to validate our framework are presented in \autoref{section:3dmuscleexps}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Muscles and Hill's model}\label{section:3dmusclephysiologyhill}
In this section we provide a short description of the physiology of skeletal muscles and a brief discussion on the Hill-type muscle model.
\subsection{Physiology of skeletal muscles}\label{section:3dmusclephysiology}
Skeletal muscles contain several tissues, including fibres, connective tissue, blood vessels, nerves, intra and extracellular matrix, among others. From a macroscopic point of view, fibres are considered the smallest units in muscles. These fibres are long and cylindrical cells composed by {\it sarcomeres} arranged in parallel. In these sarcomeres, muscle fibres are activated through electrochemical processes that start from the brain and end in the nerves within the muscle: these processes produce forces inside the sarcomeres which stretch them from their resting position. Passive elastic forces are inherent to the sarcomeres, nonlinearly preventing them from lengthening. The space between muscle fibres is filled by the endomysium. The perimysium wraps groups of muscle fibres to form {\it fascicles}. Muscle are composed by fascicles that are arranged in parallel. The epimysium wraps around the fascicles and constitutes the most external layer of connective tissue in muscles. Blood vessels run in between fascicles while the ends of the nerves enter the connective tissue, branch around the muscle, and connect with the sarcomeres inside the muscle fibres.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = 1.0\textwidth, height=0.4\textheight]{muscle_structure.jpg}
    \caption{Structure of a skeletal muscle \cite{ref:nih2018}.}
    \label{fig:3dmuscleskeletalmuscle}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Hill-type muscle model}\label{section:hillmodel}
Hill's model, named after A. V. Hill who introduced it in \cite{ref:hill1938}, is widely utilized in biomechanics to estimate the force produced by a muscle during in vivo experiments when direct measurements are not available (see, e.g. \cite{ref:vanleeuwen1992,ref:richards2013}). This model provides reasonable estimates of muscle forces during slow contractions \cite{ref:dick2017} with maximal activation of the muscle fibres  \cite{ref:perreault2003,ref:wakeling2012}. 
The model assumes muscles behave as one dimensional nonlinear damper-spring systems with an extra element referred to as the {\it contractile element}. The forces generated by a muscle during contraction are then described by the following equation:
\begin{align*}
    F_{mus}(\lambda,\epsilon) := F_0(a(t)\hat{F}_{act}(\lambda,\epsilon)+\hat{F}_{pas}(\lambda)),
\end{align*}
where $\hat{F}_{act}$ is the muscle force due to the activation of the muscle fibres (contractile element force), $\hat{F}_{pas}$ is the nonlinear elastic force (passive elastic element), usually referred to as the {\it passive force}, $F_0$ is the maximum isometric force of muscles, $\lambda$ is the one dimensional stretch, and $\epsilon$ is the rate of change of the stretch over time, commonly referred to as the {\it strain rate}. The function $a = a(t)\in[0,1]$ represents the activation level of the muscle fibres over time. The definitions of the active and passive forces are normalized to the maximum isometric force $F_0$.

The active forces in Hill's model are due to the activation of the sarcomeres within muscle fibres, which causes the fibres to generate force. A key assumption in Hill's model is that these forces depend on both the length and velocity at which the fibres are being stretched. The form of the active forces is given by
\begin{align}
    \hat{F}_{act}(\lambda,\epsilon) = \hat{F}_{len}(\lambda)\hat{F}_{vel}(\epsilon),
\end{align}
where $\hat{F}_{len}$ are the forces generated from length changes in the muscle and $\hat{F}_{vel}$ are the forces due to the changes in the strain rate. The force $\hat{F}_{vel}$ satisfies $\hat{F}_{vel}(0) = 1$. The forces $\hat{F}_{len}$ and $\hat{F}_{vel}$ are defined as nonlinear functions of the stretch $\lambda$ and the strain rate $\epsilon$ respectively, as seen in \autoref{fig:3dmuscleactive-passive}. These are commonly called {\it force-length} and {\it force-velocity} relationships.

In this model, isometric contractions of muscles are considered as steady-state processes where the strain rate is assumed to be zero. This means that the active forces are only due to changes in the length of the muscle, that is
\begin{align*}
    \hat{F}_{act}(\lambda,0) = \hat{F}_{len}(\lambda).
\end{align*}
Passive forces $\hat{F}_{pas}$ act to resist fibres from stretching to longer lengths. These play an important role in muscle contraction as nonlinear springs: when muscle fibres are lengthened, nonlinear passive forces are produced to shorten the fibre back. However, when fibres contract to shorter lengths, experimental data suggest that no passive forces act to lengthen them back to their initial lengths (see \autoref{fig:3dmuscleactive-passive}); see, for instance \cite{ref:ross2018-2}.

Even though Hill-type muscle models are simple and reasonably accurate in some situations, they fail to consider many features of whole muscle dynamics and actual architecture. Mass and inertial effects are not considered in most Hill-type models, and this may contribute to inaccurate muscle force predictions when the strain rate is dynamically changing. In addition, the three-dimensional architecture of muscle cannot be represented by Hill's model alone. Muscles are nearly incompressible tissues \cite{ref:baskin1967}, and thus, when muscle deforms, some parts of the surface of the muscle deform inwards while other parts outwards, even during isometric contractions \cite{ref:wakeling2020,ref:ryan2020}. Besides, the deformation of muscles in three dimensions also depends on other tissues not explicitly considered in Hill's model; tendon, aponeurosis, base material, and fat all affect the dynamics and mechanics of muscles \cite{ref:rahemi2015,ref:ross2018-2}. Therefore, to be able to better capture and understanding the behaviour of muscle deformation in three dimensions, a more involved model is needed. The details of such a model are presented in \autoref{section:3dmusclemethods}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The mechanics of skeletal muscles}\label{section:3dmusclemechanics}
Let us start by recalling some basic concepts in the theory of nonlinear elasticity. This overview is mainly based on \cite{ref:ogden1997,ref:volokh2016}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Nonlinear continuum mechanics}\label{section:3dmusclenonlinear}
Suppose that an elastic body initially occupies a bounded region $V_0\subseteq\rrr^3$. 
We consider, for fixed $t>0$, that there exists a diffeomorphism $\phi(\cdot,t):V_0\to V$ which maps every point in $V_0$ onto a bounded region  
$V\subseteq\rrr^3$, that is the range of $\phi(\cdot,t)$ is exactly $V$. The region $V_0$ is referred to as the initial configuration on the elastic body while $V$ represents the current configuration of such body. We assume that this map is such that $\phi(\cdot,0)$ is the identity function. We also use the notation $\phi_t(\cdot) = \phi(\cdot,t)$. Thus, a point $\x\in V$ can be written 
as $\x = \phi(\x_0,t)$, for some $\x_0\in V_0$ (see \autoref{fig:3dmuscleconfigurations}). We define the {\it displacement} of the point $\x_0\in V_0$ at time $t>0$ as
\begin{align*}
 \u(\x_0,t) := \x - \x_0 = \phi(\x_0,t) - \x_0.
\end{align*}
The {\it velocity} at which the point $\x\in V$ is changing at time $t>0$ is simply defined as 
\begin{align*}
 \v := \frac{\partial \u}{\partial t},
\end{align*}
where $\frac{\partial}{\partial t}$ denotes the time derivate in the current configuration $V$.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = 1\textwidth,  height=.35\textheight]{initialcurrentconfig.png}
    \caption{Sketch of the initial and current configurations, and the map $\phi$.}
    \label{fig:3dmuscleconfigurations}
\end{figure}
Note that we can differentiate the displacement $\u$ with respect to spatial variables in both $V_0$ or $V$ for any fixed $t>0$. From here on, the differential operator $\nabla$ will be employed to denote the gradient of a function defined in the current configuration $V$. The operator $\div$ coincides with the trace of the tensor defined by $\nabla$. The divergence operator for tensors, denoted by $\bdiv$, is defined as the divergence operator $\div$ acting on each row of tensors.
On the initial configuration $V_0$ we add the subscript $0$ to the differential operators above to denote them, that is $\nabla_0$, $\div_0$, and $\bdiv_0$, as differential operators in $V_0$. With this notation, the {\it deformation tensor} $\ff(\x_0,t)$ is defined from the displacement $\u$ by 
\begin{align*}
 \ff(\x_0,t) := \ii + \nabla_0\u(\x_0,t),\,\,\x_0\in V_0,\,\,t>0.
\end{align*}
The inverse of the deformation tensor is given by the gradient of the displacement in the current configuration $V$:
\begin{align*}
    \ff^{-1} = \ii - \nabla\u,\,\, t>0.
\end{align*}
The dilation of such a deformation defines the infinitesimal volume changes of 
$V_0$ over time and is defined by
\begin{align}
    J(\x_0,t) := \det(\ff(\x_0,t)).\label{eq:3dmuscledilation}
\end{align}
This dilation is assumed to be strictly positive. A deformation of the body such that $J\in(0,1)$ indicates that the local volume is decreasing, while a dilation $J$ greater than 1 indicates that the local volume is increasing. The particular case in which $J = 1$ indicates that no local changes in volume occur during deformation and occurs when the deformation is assumed to be incompressible. Negative or zero dilations result in deformations in which the current volume is negative or zero. Both the dilation and the deformation tensor provide the following change of variables between $V$ and $V_0$ as well as between their surfaces:
\begin{align}
    \int_{V}f(\x) = \int_{V_0} J(\x_0,t) f_0(\x_0),\quad \int_{\partial V} f(\x)\n = \int_{\partial V_0} J(\x_0,t)\,\ff(\x_0,t)^{-\transpose}f_0(\x_0)\n_0,\quad\forall\,t>0.\label{eq:3dmusclechangevariables}
\end{align}
The functions $f_0$ and $f$ are defined over $V_0$ and $V$ respectively, and are related by $f_0 := f\circ\phi_t$. Here $\n_0$ and $\n$ denote the outward unit normal vector on $\partial V_0$ and $\partial V$ respectively. The change of variables over the surface is a consequence of Nanson's formula (see, e.g. \cite{ref:ogden1997}).

We assume the mass in $V_0$, denoted by $m(V_0)$, is conserved over time. The mass of the elastic body in the current configuration $V$ is defined through its current density $\rho:V\to\rrr$, as
\begin{align*}
    m(V) = \int_{V}\rho(\x,t).
\end{align*}
Conservation of mass means that $m(V_0) = m(V)$, which is equivalent to saying that the total time derivative, denoted by $\frac{d}{dt}$, of $m(V)$ must vanish:
\begin{align}
    \frac{d}{dt}m(V) = 0\quad\forall\,t>0.\label{eq:3dmuscleconversemass}
\end{align}
The definition of the mass in $V$, together with the Reynolds transport theorem and the divergence theorem, yield the following equation for the conservation of mass in $V$:
\begin{align}
    \frac{\partial\rho}{\partial t} + \rho\,\div\,\v = 0\quad\text{in $V$}.\label{eq:3dmusclebalancemass}
\end{align}
Note that the condition $m(V_0) = m(V)$ also implies that
\begin{align*}
    \int_{V_0} \rho_0(\x_0) = \int_V \rho(\x,t),\quad\forall\,t>0,
\end{align*}
where $\rho_0:V_0\to\rrr$ represents the density of the body in the initial configuration $V_0$. Using the changes of variables of volume integrals given in \eqref{eq:3dmusclechangevariables} we have the relation
\begin{align}
    \rho = \frac{1}{J}\rho_0,\quad\forall\,t>0.
\end{align}
The linear momentum of the elastic body in $V$ is given by
\begin{align}
    \ell(V,t) = \int_V\rho(\x,t)\,\v(\x,t),\label{eq:3dmusclelinearmomentum}
\end{align}
whereas the angular momentum of the body in $V$ about a fixed point $\p\in\rrr^3$ is defined as
\begin{align}
    \omega(V,\p,t) := \int_V\rho(\x,t)\,(\x-\p)\times\,\v(\x,t),\label{eq:3dmuscleangularmomentum}
\end{align}
with "$\times$" denoting the usual cross product of vectors in $\rrr^3$. Given $t>0$, consider a body force $\b(\cdot,t)\in\ll^2(V)$, and a prescribed traction $\t(\cdot,t)\in\ll^2(\partial V)$. The balance of linear and angular momenta of the elastic body in $V$ can be written as
\begin{subequations}\label{eq:3dmusclebalancemomenta}
\begin{align}
    \frac{d}{dt}{\ell}(V,t) &= \int_V\b(\x,t) + \int_{\partial V}\t(\x,t),\label{eq:3dmusclebalancelinearmomentum}\\
    \frac{d}{dt}{\omega}(V,\p,t) &= \int_V(\x-\p)\times\,\b(\x,t) + \int_{S_N}(\x-\p)\times\,\t(\x,t).\label{eq:3dmusclebalanceangularmomentum}
\end{align}
\end{subequations}
Cauchy's theorem (see, e.g., \cite{ref:ogden1997}) states that there exists a second order tensor $\bsigma$ such that the traction $\t$ depends linearly on the normal unit vector on $\partial V$, that is
\begin{align}
    \t = \bsigma\,\n\quad\text{on $\partial V$}.
\end{align}
Such a second order tensor $\bsigma$ is referred to as the {\it Cauchy stress tensor}. The balance of angular momentum in \eqref{eq:3dmusclebalanceangularmomentum} implies the symmetry of this tensor, that is
\begin{align}
    \bsigma^\transpose = \bsigma\quad\text{in $V$}.\label{eq:3dmusclesymmcauchytensor}
\end{align}
On the other hand, the balance of linear momentum in \eqref{eq:3dmusclebalancelinearmomentum} provides us with the following balance of forces in the current configuration:
\begin{align}
    \rho\,\frac{D\v}{Dt} = \bdiv(\bsigma^\transpose) + \b\quad\text{in $V$},\label{eq:3dmusclebalanceforces}
\end{align}
where $\frac{D}{Dt}$ denotes the time derivative in the initial configuration $V_0$ or the {\it material derivative}. We can combine \eqref{eq:3dmusclebalancemass}, \eqref{eq:3dmusclesymmcauchytensor}, and \eqref{eq:3dmusclebalanceforces}, and use the definition of the material derivative $\frac{D}{Dt}(\cdot) = \frac{\partial}{\partial t}(\cdot) + \v\cdot\nabla(\cdot)$ to obtain the following balance of forces:
\begin{align}
    \frac{\partial(\rho\,\v)}{\partial t} + \bdiv(\rho\,\v\otimes\v) = \bdiv(\bsigma) + \b\quad\text{in $V$}.\label{ref:forcebalance}
\end{align}
For compressible materials, it is useful to split the Cauchy tensor into a volume 
preserving (or isochoric) and a volume changing component (see, e.g. \cite{ref:wriggers2009,ref:volokh2016}). As we shall see in the next section, the volumetric component of the Cauchy tensor will depend on the dilation $J$, while the isochoric component will depend on both the displacement $\u$ and velocity $\v$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Skeletal muscle mechanics}\label{section:3dmusclemuscle}
\sebacomments{Need to rephrase this section.} 
Our definition of the Cauchy stress tensor not only depends on the displacement, but also depends on the internal pressure, the dilation, and the velocity. 

The Cauchy stress tensor $\bsigma$ is conformed of various components, each of them encoding different properties of a particular tissue or material. The assumption that muscles are nearly incompressible tissues can be translated into a split of the Cauchy tensor: a volumetric part, denoted by $\bsigma_{vol}$, and an isochoric (or isovolumetric) part, denoted by $\bsigma_{iso}$. The change in volume during the deformation of the tissues implies the change in internal pressure, which we denote by $p$. In this way, the volmetric part of the Cauchy tensor, $\bsigma_{vol}$ depends on both the dilation $D$ and the pressure $p$. The variable $D$ is defined as the true dilation $J(\u)$ in the current configuration through the use of a Lagrange multiplier, that is
\begin{align*}
    D = J(\u)\quad\text{in $V$}.
\end{align*}
On the other hand, the isochoric part of the Cauchy tensor, $\bsigma_{iso}$ encloses the properties of incompressible deformations. Equivalently this indicates that stresses due to volume changes are not considered in the definition of $\bsigma_{iso}$ but instead are encapsulated in the definition of the isovolumetric Cauchy stress tensor $\bsigma_{vol}$. In general, however, the isochoric Cauchy stress tensor depends on the displacement $\u$. In addition, to be able to account for the contribution from the force-velocity relationship in Hill's model, we additionally assume that $\bsigma_{iso}$ depends on the velocity $\v$, which in some way we are to see later, related to the fibre velocity. Thus we can write the split of the Cauchy stress tensor as follows:
\begin{align}
    \bsigma(\u,\v,p,D) = \bsigma_{vol}(p,D) + \bsigma_{iso}(\u,\v).
\end{align}
The usual definition of the pressure in the literature is through the Cauchy stress tensor itself, with $p = -\frac{1}{3}\tr(\bsigma)$. In this study we make use of a different definition for such a pressure, based on the work in \cite{ref:simo1985,ref:pelteret2012}. In this work the pressure is defined in terms of the dilation as
\begin{align*}
    p = \frac{\kappa}{2}\Big(D-\frac{1}{D}\Big)\quad\text{in $V$}.
\end{align*}

Note that the definition of the pressure as $p = \Psi_{vol}'(D)$ slightly differs from the usual definition of $p = -\frac{1}{3}\tr(\bsigma)$. However, we see that the pressure we compute is actually much closer to the classical definition. Due to the split in the strain energies densities, we see that the Cauchy tensor can be written as
\begin{align*}
    \bsigma = p\ii + \bsigma^\deviator,
\end{align*}
where $\bsigma^\deviator := \bsigma - \frac{1}{3}\tr(\bsigma)\ii$ is the deviator of the tensor $\bsigma$. Thus, taking trace on the definition of the Cauchy tensor above one finds
\begin{align*}
    p = \frac{1}{3}\tr(\bsigma).
\end{align*}
Thus, in our model we compute the classical pressure with opposite sign.

Let us consider the Helmholtz free energy $\Psi$ of skeletal muscle tissues confined to the region $V_0$ in $\rrr^3$. We assume the energy is split into a volume preserving and a volume changing parts as follows:
\begin{align*}
    \Psi = \Psi_{vol}(J) + \Psi_{iso}(\u,\v),
\end{align*}
where the displacement $\u$, the velocity $\v$, and the dilation $J$ are defined as in the previous section.

In our model we assume that the volumetric part of the free energy $\Psi_{vol}$ only depends on the dilation $J$ and is such that $\Psi_{vol}(1) \equiv 0$. In particular, this means that no energy due to volume changes are considered if the tissues are incompressible. In this study we adopt the form of the volumetric energy used in \cite{ref:pelteret2012,ref:rahemi2014} (see also \cite{ref:holzapfel2001} for more details on volume changing free energy functions). The volumetric part of the free energy is defined as
\begin{align*}
    \Psi_{vol}(J) := \frac{\kappa_{tis}}{4}\big(J^2-2\log(J)-1\big),\,\,
    tis\in\{mus,apo,ten\},
\end{align*}
in which $\kappa_{tis}>0$ is the bulk modulus of the corresponding tissue, and {\it mus}, ${\it apo}$, and ${\it ten}$ refer to muscle, aponeurosis, and tendon respectively. In turn, the volume preserving (or isochoric) part of the energy $\Psi_{iso}$ depends on both the displacement and the velocity.

As described previously, our model of skeletal muscle consists mainly of muscle, tendon, aponeurosis, and base material. We consider muscle, aponeurosis, and tendon as anisotropic fibre-reinforced composite and nearly incompressible materials \cite{ref:rahemi2014}. The tissues are composed mostly of one dimensional curvilinear fibres running from one point to another within $V_0$. However, the space between fibres is not empty. Among the different materials that comprise the base material, the most abundant is collagen \cite{ref:zatsiorsky2012}. As in \cite{ref:rahemi2014}, we assume that this material is isotropic. We consider the following split of the isochoric free energy:
\begin{align*}
    \Psi_{iso}(\u,\v) := \Psi_{base,tis}(\bar\bb) + \Psi_{tis}(\bar\lambda,\bar\epsilon),\,\,\,tis\in\{mus,apo,ten\},
\end{align*}
where $\bar\bb := J^{-2/3}\bb$, $\bar\lambda := J^{-1/3}\lambda$, and $\bar\epsilon$ is the strain rate of the fibres (muscle and collagen) in the different tissues. The variable $\lambda$ is usually referred to as the stretch in the fibre, which quantifies the lengthening and shortening of a given fibre. Following \cite{ref:simo1991}, if the unit vector $\a_0\in\rrr^3$ denotes the initial orientation of a fibre at a point $\x_0\in V_0$, then the stretch of the fibre at that location is given as
\begin{align}
    \lambda := \|\ff\,\a_0\|,\label{eq:3dmuscledef-stretch}
\end{align}
where $\|\cdot\|$ denotes the usual 2-norm of vectors in $\rrr^3$. This means that the value of the stretch depends directly on the deformation of the fibre. As explained above, the deformation tensor provides a change of variables from the initial onto the current configuration. In particular, the vector $\a:=\ff\,\a_0$ denotes the orientation vector of the deformed fibre which has an orientation $\a_0$ at the point $\x_0$ in $V_0$. Thus, $\a$ is the orientation of the same fibre in the current configuration $V$. Similarly, the variable $\bar\epsilon$ is the strain rate of the fibre. This says that $\bar\epsilon$ is the velocity at which the fibre is being stretched per unit of time. In this work we define the strain rate as the velocity at which the displacement is changing in the along fibre direction. Therefore, the strain rate can be written as
\begin{align}
    \bar\epsilon := \v\cdot\a.\label{eq:3dmuscledef-strainrate}
\end{align}
The free energy defining the mechanical responses of the base material of the different tissues is defined as \cite{ref:yeoh1993}
\begin{align*}
     \Psi_{base,tis}(\bar\bb) := %\begin{cases}
    s_{base,tis}\sum_{k=0}^3 c_k(\tr(\bar\bb)-3)^k,\quad tis\in\{mus,apo,ten\},
    % , & \text{for muscle \cite{ref:yeoh1993}},\\ c_4(\exp(c_5(\tr(\bar\bb)-3))-1), & \text{for aponeurosis \cite{ref:humphrey1987}},\\
    %         %5.256\rme5 \cdot
    %         c_6(\tr(\bar\bb) - 3), & \text{for tendon \cite{ref:humphrey1987}},
    %                           \end{cases}
\end{align*}
where the constants $c_k\in\rrr$, $k=0,\ldots,3$, are to be determined based on experimental data \cite{ref:}. The constant $s_{base,tis}>0$ is added to the definition of the base material strain energy to change the stiffness of the material as needed. 

Even though the general formulation of the free energy $\Psi_{tis}$ depends on both the stretch and the strain rate in the fibres, only muscle fibres possess stresses depending on both of these. For aponeurosis and tendon, the free energy $\Psi_{tis}$ depends only on $\bar\lambda$. The stress $\sigma_{mus}$ for muscle is assumed to have the form
\begin{align}
    \sigma_{mus}(\bar\lambda,\bar\epsilon) = \sigma_0\big(\hat{\sigma}_{act}(\bar\lambda,\bar\epsilon) + \hat{\sigma}_{pass}(\bar\lambda)\big),
\end{align}
where $\sigma_0>0$ is the maximum isometric stress in the muscle fibres, $\hat{\sigma}_{act}$ is the active stress and $\hat{\sigma}_{pass}$ is the passive stress in the fibre. In this work we adopt the function representation in \cite{ref:ross2018-2}, which is based on cubic Bezier curves \cite{ref:ross2018-1}. 

In general, the active stress is defined by two forces of different nature: elastic forces due to the stretch of the muscle fibres and forces due to the velocity at which the muscle fibres are being stretched. similar to the definition of active forces in the Hill-type muscle model, the active stress is defined as
\begin{align*}
    \hat{\sigma}_{act}(\bar\lambda,\bar\epsilon) := \hat{\sigma}_{len}(\bar\lambda)\hat{\sigma}_{vel}(\bar\epsilon).
\end{align*}
Here $\hat{\sigma}_{len}$ is called the force-length function whereas $\hat{\sigma}_{vel}$ is the force-velocity function (see \autoref{fig:3dmuscleactive-passive}). For the sake of clarity, in this case the velocity refers to the velocity in which the fibres are stretched, that is, it is simply the strain rate $\bar\epsilon$. By looking at \eqref{eq:3dmuscledef-strainrate}, we see that, in general, they do not coincide. We remark that both $\sigma_{ten}$ and $\sigma_{apo}$ depend only on the stretch in the fibres $\bar{\lambda}$. 

\graphicspath{{../images/}}
\begin{figure}[!ht]
\centering\includegraphics[width = 1\textwidth, 
height=0.4\textheight]{ActivePassiveCurves.pdf}
\caption{Force-velocity (left), force-length and passive stress (right) functions used in this study.}\label{fig:3dmuscleactive-passive}
\end{figure}

% \sebacomments{ADD tissue properties!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem formulation}\label{section:3dmuscleformulation}
Let $S$ be a non-empty subset of $\partial V$ with positive measure. Let us first recall some equations from \eqref{eq:3dmusclebalancemass}, \eqref{eq:3dmusclesymmcauchytensor}, and \eqref{eq:3dmusclebalanceforces}:
\begin{subequations}\label{eq:3dmusclebalance}
\begin{align}
    \frac{\partial\u}{\partial t} = \v,\label{eq:3dmusclebalance1}\\
    \frac{\partial\rho}{\partial t} + \div(\rho\,\v) = 0,\label{eq:3dmusclebalance2}\\
    \bsigma^\transpose = \bsigma,\label{eq:3dmusclebalance3}\\
    \rho\,\frac{D\v}{Dt} = \bdiv(\bsigma^\transpose) + \b.\label{eq:3dmusclebalance4}
\end{align}
\end{subequations}
Since our model considers nearly incompressible tissues, we add the dilation to the system as a new unknown via a Lagrange multiplier. In this case, the internal potential energy in $V$ becomes
\begin{align}
    U(\u,\v,p,D) := \int_{V}\Psi_{vol}(D) + p\,(J(\u)-D) + \Psi_{iso}(\u,\v),\label{eq:3dmusclepotential}
\end{align}
where the Lagrange multiplier $p$ denotes the internal pressure in the tissues. Let $t>0$ be given. The problem of large deformation of skeletal muscles is formulated as follows: given an initial displacement $\u_0\in\hh^1(V_0)$, velocity $\v_0\in\hh^1(V_0)$, pressure $p_0\in L^2(V_0)$, dilation $D_0\in L^2(V_0)$, body force $\b(\cdot,t)\in\ll^2(V)$, known traction $\t(\cdot,t)\in\hh^{-1/2}(\partial V\backslash S)$, and prescribed displacement $\d(\cdot,t)\in\hh^{1/2}(S)$, we want to find large deformations $\u(\cdot,t)\in\hh^1(V)$, internal pressure $p(\cdot,t)\in L^2(V)$, and dilation $D(\cdot,t)\in L^2(V)$ such that
\begin{subequations}\label{eq:3dmuscleeqs-muscle}
\begin{align}
 \frac{\partial\u}{\partial t} = \v,\,\,\frac{\partial(\rho\v)}{\partial t} + \bdiv(\rho\,\v\otimes\v)= \bdiv\,\bsigma(\u,\v,p,D) + \b\,\,\mbox{in $V$},\label{eq:3dmuscleeqs-muscle1}\\
 D-J(\u) = 0,\,\, p-\Psi_{vol}'(D) = 0,\,\,\mbox{in $V$},\label{eq:3dmuscleeqs-muscle2}\\
 \mm\u = \d,\,\,\mbox{on $ S $},\,\,\bsigma(\u,\v,p,D)\,\n = \t,\,\,\mbox{on $\partial V\backslash S $},\\
 \u = \u_0,\quad \v = \v_0,\quad p = p_0,\quad D = D_0,\quad\text{in $V_0$}.\label{eq:3dmuscleeqs-muscle3}
\end{align}
\end{subequations}
Here the tensor $\mm\in\lll^\infty( S )$ is added to allow the implementation of more general boundary conditions (such as gliding boundary conditions). 

Note that the definition of the pressure as $p = \Psi_{vol}'(D)$ slightly differs from the usual definition of $p = -\frac{1}{3}\tr(\bsigma)$. However, we see that the pressure we compute is actually much closer to the classical definition. Due to the split in the strain energies densities, we see that the Cauchy tensor can be written as
\begin{align*}
    \bsigma = p\ii + \bsigma^\deviator,
\end{align*}
where $\bsigma^\deviator := \bsigma - \frac{1}{3}\tr(\bsigma)\ii$ is the deviator of the tensor $\bsigma$. Thus, taking trace on the definition of the Cauchy tensor above one finds
\begin{align*}
    p = \frac{1}{3}\tr(\bsigma).
\end{align*}
Thus, in our model we compute the classical pressure with opposite sign.

In \autoref{section:3dmusclemethods} we introduce the numerical scheme to approximate the solutions of the nonlinear system in \eqref{eq:3dmuscleeqs-muscle}. A semi-implicit time stepping is applied at the continuous level to discretize the time variable. The nonlinear equations are solved via the application of a Newton's iteration. Finally we discretize the space variables of the resulting linear system with a mixed FEM.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical approach}\label{section:3dmusclemethods}
To approximate a solution of the nonlinear dynamic system in \eqref{eq:3dmuscleeqs-muscle}, we use a semi-implicit time stepping for the time derivatives, and a conforming finite element scheme for the spatial variables. The displacement, 
dilation, and pressure are updated with an implicit approach while the velocity is computed with an explicit update. The velocity is treated explicitly and it is only updated once the new displacement is computed.
Using this time stepping in \eqref{eq:3dmuscleeqs-muscle}, we propose
\begin{align*}
 \u^{n+1} - \delta t\v^{n+1} = \u^n,\\
 \rho^{n+1}\v^{n+1} - \delta t\cdot\bdiv\,\bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1}) = \rho^n\v^n -\delta t\cdot\bdiv(\rho^n\v^n\otimes\v^n) + \delta t\b^{n+1},\\
 D^{n+1} - J(\u^{n+1}) = 0,\,\,p^{n+1} - \frac{\partial\Psi_{vol}}{\partial D^{n+1}} = 0,\\
 \bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1})\n = \t^{n+1},\,\, \mm\u^{n+1} = \d^{n+1},
\end{align*}
where $\delta t>0$ is the time step size. Combining the first two equations above we can get
\begin{align*}
 \rho^{n+1}\u^{n+1} - \delta t^2\cdot\bdiv\,\bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1}) =&\,\rho^{n+1}\u^n+\delta t\cdot\rho^n\v^n \\
 &+ \delta 
t^2\cdot\big(-\bdiv(\rho^n\v^n\otimes\v^n)+\b^{n+1}\big),\\
 D^{n+1} - J(\u^{n+1}) = 0,\quad &p^{n+1} - \frac{\partial\Psi_{vol}}{\partial D^{n+1}} = 0,\\
 \bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1})\n = \t^{n+1}&,\quad \mm\u^{n+1} = \d^{n+1}.
\end{align*}
Multiplying these equations by a test function $\bchi:=(\w,q,H)\in\xx:=\hh^1(V)\times L^2(V)\times L^2(V)$ and 
integrating by parts one obtains the nonlinear problem: given the previous displacement $\u^n$, previous velocity $\v^n$, force $\b^{n+1}$, 
traction $\t^{n+1}$, and prescribed displacement $\d^{n+1}$, we are to find $\bxi^{n+1}:=(\u^{n+1},p^{n+1},D^{n+1})\in\xx$ such that
\begin{align}
 a_{\v^n}(\bxi^{n+1},\bchi) = F_{\u^n,\v^n}(\bchi),\,\,\forall\,\bchi\in\xx,\label{eq:3dmusclemuscleweakform}
\end{align}
where the map $a_{\v^n}:\xx\times\xx\to\rrr$ and the functional $F_{\u^n,\v^n}:\xx\to\rrr$ are defined by
\begin{align*}
 a_{\v^n}(\bxi^{n+1},\bchi) &:=\, \big(\rho^{n+1}\u^{n+1},\w\big)_{V} \\
&+\delta t^2\cdot\Big\{\big(\bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1}),\nabla\w\big)_{V}\\
&+\big(p^{n+1}-\frac{\partial\Psi_{vol}}{\partial D^{n+1}},q\big)_{V} + 
\big(D^{n+1}-J(\u^{n+1}),H\big)_{V}\Big\},\\
F_{\u^n,\v^n}(\bchi) &:= \,\big(\rho^{n+1}\u^n,\w\big)_{V}+\delta t\cdot\big(\rho^n\v^n,\w\big)_{V}-\delta t^2\cdot\big( 
\bdiv(\rho^n\v^n\otimes\v^n),\w\big)_{V}\\
&+ \delta t^2\cdot\Big\{\big( 
\b^{n+1},\w\big)_{V} + \big( 
\t^{n+1},\w\big)_{\partial V\backslash S}\Big\}.
\end{align*}
The terms $\big(p^{n+1}-\frac{\partial\Psi_{vol}}{\partial D^{n+1}},q\big)_{V}$ and $\big(D^{n+1}-J(\u^{n+1}),H\big)_{V}$ are multiplied by $\delta t^2$ to obtain a symmetric linear system to solve after a linearization of 
\eqref{eq:3dmusclemuscleweakform}. Assuming $\u^n$ and $\v^n$ belong to $\ll^2(V)$, the $F_{\u^n,\v^n}$ is a linear and bounded functional in $\xx$. On the other hand, we note that the map $a_{\v^n}$ is linear only in the second argument. We remark that problem in \eqref{eq:3dmusclemuscleweakform} is well-defined as long as the Cauchy stress tensor 
$\bsigma(\u^{n+1},\v^n,p^{n+1},D^{n+1})$ belongs to $\lll^2(V)$. 

Note that the integrals over the current configuration $V$ can be transformed into integrals over $V_0$ by using the change of variables given in \eqref{eq:3dmusclechangevariables}. The advantage of considering this change of variables is that we do not need to save all the necessary information to build a mesh of $V$ at every time step. This would also require meshing the current configuration at every time step. Integrating over the initial configuration avoids this issue which translate to efficiencies in computing time. We only need to keep track of variables that are needed to apply the changes of variables in \eqref{eq:3dmusclechangevariables}: these are the dilation, deformation tensor, and the updated weights for the corresponding quadrature rule.

The nonlinear nature of this problem can be handled with a Newton's iteration. Given the previous displacement $\u^n$ and previous velocity $\v^n$, we define the residual operator 
$R_{\u^n,\v^n}:\xx\to\xx^*$ as
\begin{align}
 [R_{\u^n,\v^n}(\bxi^{n+1}),\bchi]_\xx := a_{\v^n}(\bxi^{n+1},\bchi) - F_{\u^n,\v^n}(\bchi),\label{eq:3dmuscleresidual}
\end{align}
where $[\,\cdot\,,\,\cdot\,]_\xx$ denotes the duality pairing between $\xx$ and $\xx^*$. Thus, if we assume we know a solution $\bxi^n\in\xx$ and a velocity $\v^n\in\hh^1(\Omega)$ at time step $t_n>0$, $n\in\nnn$, the Gateaux derivative for bounded functionals gives the following system: provided we have found the state $\bxi_k\in\xx$, $k\geq0$, we want to obtain a new state 
$d\bxi:=(d\u,dp,dD)\in\xx$ such that
\begin{align}
 \big[\dddd R_{\v^n}(\bxi_k)(d\bxi),\bchi\big]_\xx = -\big[R_{\u^n,\v^n}(\bxi_k),\bchi\big]_\xx,\quad\forall\,\bchi\in\xx,\label{eq:3dmusclelinearform}
\end{align}
where the Gateaux derivative $\dddd R_{\v^n}(\bxi_k)$ has the following saddle-point structure
\begin{align*}
    \left[\begin{array}{ccc}
        \begin{array}{c}
 (\rho_0\,d\u,\w)_{V_0} + \delta t^2\cdot(\btau_k\nabla d\u,\nabla\w)_{V_0}  \\
             + \delta t^2\cdot(\ccc_k\,\nabla d\u,\nabla\w)_{V_0}
        \end{array} & \delta t^2\cdot(D_k\,q,\div d\u)_{V_0} & 0 \\
        & & \\
        \delta t^2\cdot(D_k\,dp,\div\w)_{V_0} & 0 & -\delta t^2\cdot(dp,H)_{V_0} \\
        & & \\
        0 & -\delta t^2\cdot(q,dD)_{V_0} & \delta t^2\cdot(\Psi_{vol}''(D_k)dD,H)_{V_0}
    \end{array}\right],
\end{align*}
where $\ccc_k = 2\frac{\partial\ss_k}{\partial\cc_k}$ is the 4th order elasticity tensor, $\ss$ is the first Kirchhoff tensor, and $\cc$ is the left Cauchy tensor. We note that the Piola-Kirchhoff tensor $\btau_k$ and the 4th order tensor $\ccc_k$ depend only on the previous state $\bxi_k$ and the velocity at the previous time step $\v^n$, whereas the term $\Psi_{vol}''$ only depends on the dilation given by the previous state $\bxi_k$. This implies that the operator $\dddd R_{\v^n}(\bxi_k)$ is linear in both $d\bxi$ and $\bchi$. 

After solving the system in \eqref{eq:3dmusclelinearform}, we set the next iterate as $\bxi_{k+1} := \bxi_k + d\bxi$ and check the norm of $R_{\u^n,\v^n}(\bxi_{k+1})$. Since we want to find zeros of \eqref{eq:3dmuscleresidual}, the stopping criteria is simply a small tolerance for the norm of the residual operator. To initiate the nonlinear iteration in \eqref{eq:3dmusclelinearform} we put $\bxi_0 = \bxi^n$. When the stopping criteria is met we define $\bxi^{n+1} := \bxi_K$, where $K\in\nnn$ denotes the last iteration of the Newton's iteration.

Even though all integrals are taken over $V_0$, the gradients of the unknowns and test functions are computed in the current configuration $V$. However, the change of variables
\begin{align*}
    \nabla\w = \nabla_0\w\,\ff^{-1},\,\,\w\in\hh^1(V_0),
\end{align*}
is applied in our implementation to obtain the gradients in the current configuration from gradients of basis functions defined only on $V_0$.

The main advantage of writing the operator $\dddd R_{\v^n}(\bxi_k)$ as before is that it remains a symmetric operator. 
This makes the computation cheaper since faster iterative methods (such as preconditioned CG) can be applied to solve the corresponding linear system.

To discretize the linear operator $\dddd R_{\v^n}(\bxi_k)$ in space, we utilise a standard  conforming FEM. Let $\tttt_h$ be a regular triangulation of $\overline{V}_0$ by tetrahedra $T$ of diameter $h_T$. The meshsize $h$ is defined by $h:=\max\{h_T:\,T\in\tttt_h\}$.
We use the same finite element spaces as those used in \cite{ref:pelteret2012}: the displacements are discretized with continuous polynomials whereas the pressure and dilation are discretized with discontinuous polynomials. Note that, given the form of the operator $\dddd R_{\v^n}(\bxi_k)$, a condition between these polynomial spaces must be met is usual of mixed finite element methods. In this way, for a non-negative integer $k$ and 
an element $T$ of $\tttt_h$, let us consider $P_k(T)$ as the space of all polynomials of degree at most $k$ defined in  $T$. The space $\pp_k(T)$ would denote the vector version of $P_k(T)$. Consider the finite element spaces for $\hh^1_{\Gamma_0}(V_0)$ and $L^2(V_0)$ as 
\begin{align*}
 \qq_{k+1} &:= \big\{\w\in\cc(\overline{V}_0):\,\v|_T\in\pp_{k+1}(T),\,\,\forall\,T\in\tttt_h\big\} \cap \hh^1_{\Gamma_0}(V_0),\\
 P_k &:= \big\{q\in L^2(V_0):\,q|_T\in P_k(T),\,\,\forall\,T\in\tttt_h\big\}.
\end{align*}
We note that this choice of discrete spaces guarantees the condition $\div\,\qq_{k+1}\subseteq P_k$ for any $k\geq0$.

The discrete formulation of \eqref{eq:3dmusclelinearform} is then as follows: given the state $\bxi_{h,k}\in\xx_h$, a previous displacement $\u^n$, and a previous velocity $\v^n$, we are to find $d\bxi_h\in\xx_h:=\qq_{k+1}\times P_k\times P_k$ such that
\begin{align}
 \big[\dddd R_{\v_h^n}(\bxi_{h,k})(d\bxi_h),\bchi_h\big] = - 
\big[R_{\u_h^n,\v_h^n}(\bxi_{h,k}),\bchi_h\big],\,\,\forall\,\bchi_h\in\xx_h.\label{eq:3dmusclemusclediscreteform}
\end{align}
Since we discretize the time variable with a semi-implicit approach, we can expect that the discrete formulation in \eqref{eq:3dmusclemusclediscreteform} must obey a CFL condition. For this model the CFL condition is given by
\begin{align*}
    \|\v(\x)\|\left(\frac{\delta t}{h}\right)\leq C_{max},\quad \forall\,\x\in V,
\end{align*}
where $\|\cdot\|$ denotes the vector norm in $\rrr^3$, and $C_{max}$ is the Courant number (dimensionless), assumed to be between 0 and 1. Therefore, to ensure the stability of our computations we select the time step size $\delta t$ as
\begin{align}
    \delta t := \min\Big\{\delta t_{in},C_{max}\frac{h_{min}}{\|\v\|_{\infty,V}}\Big\},\label{eq:cflcondition}
\end{align}
where $\delta t_{in}>0$ is a given time step size (as input), $h_{min} := \min\{h_T:\,T\in\tttt_h\}$, and $\|\cdot\|_{\infty,V}$ denotes the $\ll^\infty$-norm of a vector field defined in $V$. The Courant constant $C_{max}$ is also an input of our algorithm.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical experiments}\label{section:3dmuscleexps}
In this last section we provide some numerical experiments involving quasi-static as well as dynamic contractions of muscle tissues. All experiments have been implemented in the finite element library deal.ii version 8.5.1 \cite{ref:davydov2017}. 
% A version of this code is available in the Github repository \cite{ref:dynamiccode2020}.

% The values of the parameters used in the simulations are listed in \autoref{table:3dmuscleparameters}.
% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%         \hline Parameter & Value & Parameter & Value \\\hline
%         $\sigma_0$ & $200$ kPa & $s_{base,mus}$ & $1.5$ \\
%         $c_1$ & & $s_{base,apo}$ & $1.0$ \\
%         $c_2$ & & $s_{base,ten}$ & $1.0$ \\
%         $c_3$ & & & \\\hline
%     \end{tabular}
%     \caption{Values of the parameters used in the our model.}
%     \label{table:3dmuscleparameters}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Initial conditions}\label{section:3dmuscleinitial}
The initial conditions on the displacement $\u$, pressure $p$, and dilation $J$ may not be readily available. For example, laboratory measurements can be classified in three types: {\it in vivo}, {\it in vitro} and {\it in situ}. Each of these experiments have different set-ups and, therefore different initial conditions: an {\it in vivo} experiment may experience a different internal pressure during contraction due to osmotic pressure or higher body temperature. An {\it in vitro} experiment may be performed with a muscle that has been previously frozen, changing the stiffness of the tissues.

To avoid any incompatibilities with the initial conditions, we consider simple known values of the displacement, pressure and dilation at $t=0$. First, we assume that the initial state of the tissues refers to a muscle with no deformation, including any of its rigid motions. Thus the initial condition of the displacement $\u$ is set to be the zero vector. This state with no displacement implies that the deformation tensor $\ff$ is simply the identity matrix. Hence the dilation at this state of the tissues becomes exactly 1. Finally, coming back to the definition of the pressure, we have that
\begin{align*}
    p(\x_0,0) = \Psi_{vol}'(D)\big|_{t=0} = \frac{\kappa}{2}\big(D-\frac{1}{D}\big)\big|_{t=0}.
\end{align*}
Since $D = 1$ at $t=0$, the pressure becomes zero at the initial state of the muscle. Thus, the initial conditions we use in all of the numerical simulations are
\begin{align}
    \u(\x_0,t) = \zero,\quad p(\x_0,0) = 0,\quad D(\x_0,0) = 1,\quad \x_0\in V_0.
\end{align}
Note that this choice of initial conditions is compatible with the definitions introduced in \autoref{section:3dmusclemechanics}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A convergence study}\label{section:3dmusclecv}
The first numerical test consists of a convergence study for the discrete formulation in \eqref{eq:3dmusclemusclediscreteform}. For this example, we consider a block of pure muscle tissue represented by a parallelepiped of dimensions 0.03 meters long (in the x direction), 0.01 meters wide (in the y direction), and 0.01 meters high (in the z direction). The initial configuration of the muscle is  defined as $V_0:=(-0.015,0.015)\times(-0.005,0.005)\times(-0.005,0.005)$. We define $S_0:=\{\x_0\in\overline{V}_0:x_0=-0.015\}\cup\{\x_0\in\overline{V}_0:x_0=0.015\}$. We refer to the -x face to the set $\{\x_0\in\overline{V}_0:x_0=-0.015\}$ whereas the +x face refers to the set $\{\x_0\in\overline{V}_0:x_0=0.015\}$. Muscle fibres run parallel to the x axis, with global fibre orientation vector $\a_0:=(1,0,0)^\transpose$.  

We perform the convergence study of an isometric deformation of the tissues. During isometric contractions the strain rate is set to zero, the point at which the stress $\hat{\sigma}_{vel}$ equals 1. We also assume that density and velocity effects are negligible. This is aligned with experimental data that is collected to generate force-length curves in which inertial effects and the effect of external body forces during muscle contraction are assumed to be negligible; see, for instance \cite{ref:zatsiorsky2012,ref:volokh2016}. For a fixed $t>0$ and given a traction $\t\in\hh^{-1/2}(\partial V\backslash S)$, the nonlinear system to solve is 
\begin{subequations}\label{eq:3dmuscleisometric}
\begin{align}
 \bdiv\,\bsigma(\u,\zero,p,D) = \zero,\,\,\mbox{in $V$},\,\,
 D-J(\u) = 0,\,\, p-\Psi_{vol}'(D) = 0,\,\,\mbox{in $V$},\label{eq:3dmuscleisometric1}\\
 \mm\u = \zero,\,\,\mbox{on $ S $},\,\,\bsigma(\u,\v,p,D)\,\n = \t,\,\,\mbox{on $\partial V\backslash S $},\label{eq:3dmuscleisometric2}
\end{align}
\end{subequations}
where $V$ and $S$ denote the current configurations of $V_0$ and $S_0$ respectively. First, we use a nonzero traction on the +x face to stretch the muscle fibres to a new length in the x direction, different from the initial length. Second, the -x and +x faces of the muscle block in $V_0$ are fixed in all three directions during the active contractions. 

For this example we take the following prescribed boundary conditions:
\begin{align*}
    \d = \begin{cases}
    \zero, & \text{on -x face, for all $t>0$},\\
    \zero, & \text{on +x face, for all $t_{act}\leq t\leq t_{end}$},
\end{cases}
\end{align*}
and
\begin{align*}
    \t = \begin{cases}
    \frac{p_0t}{t_{act}}(1,0,0)^\transpose, & \text{on +x face, for all $0<t<t_{act}$},\\
    \zero, & \text{on +x face, for all $t_{act}<t<t_{end}$},
\end{cases}
\end{align*}
where $p_0 = 5\cdot10^6$ Pa is a given pressure, $t_{act}$ is the start time for fibre activation, and $t_{end}$ is the end time of the simulation. The muscle fibres were activated from time $t=t_{act}$ to $t=t_{end}$. The activation function used for this example is defined as
\begin{align*}
    a(t) := \begin{cases}
    0, & \text{for all $0<t<t_{act}$},\\
    \frac{t-t_{act}}{t_{end}-t_{act}}, & \text{for all $t_{act}\leq t\leq t_{end}$}.
    \end{cases}
\end{align*}
A full list of the values of the parameters used for this run is given in \sebacomments{add full description of parameters.}
% \autoref{appendix:isometric}.

In \autoref{fig:3dmusclecvstudy} we show a convergence study of the finite element method for this experiment. This means that we are to compare the solutions within the nonlinear iterations performed by \eqref{eq:3dmusclelinearform}. We compute the errors in the $\hh^1$-norm for the Newton's update $d\u$, and in the $L^2$-norm for the Newton's update $dp$ and $dD$. The errors shown are computed at maximum activation of the fibres, that is when the activation function equals 1. We see that the each error decays with an expected rate of convergence. In fact, we note that the true solution $(d\u,dp,dD)$ belongs to $\hh^1_S(V)\times L^2(\Omega)\times L^2(\Omega)$. In addition, the convexity of the domain $V$ gives the extra regularity of the solution, which coincide with the rates of convergence shown in \autoref{fig:3dmusclecvstudy}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = 1.0\textwidth, height=0.4\textheight]{cvstudy_meshsize.jpg}
    \caption{Convergence history for the iterates $d\u$, $dp$, and  $dD$ for three different levels of refinement, at the end of the nonlinear iteration. The reference solution was computed with a $\qq_3-P_2-P_2$ scheme on a very fine mesh while the approximated solutions where computed with a $\qq_2-P_1-P_1$ scheme. The computed rate of convergence is $1.9223$ for the displacement (solid line), and $1.1299$ for both the pressure and dilation (dashed and dashed-dotted line respectively).}
    \label{fig:3dmusclecvstudy}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Dynamic contraction: cyclic contractions}\label{section:3dmuscledynamicexp}
Dynamic cyclic contractions in skeletal muscles are common during locomotion: walking, running, riding a bike or weight lifting are just a few examples of these type of contractions \cite{ref:ross2018-2}. In \cite{ref:zajac1989}, it was proposed that the time activation profile of muscle fibres, $a = a(t)$ satisfies the following ODE:
\begin{align*}
    \frac{da}{dt} + \frac{\beta+(1-\beta)u_0}{\tau_{act}}\,a = \frac{u_0}{\tau_{act}}, a(0) = 0.
\end{align*}
where $\tau_{act}$ is activation time which depends on the type of fibre (fast or slow), $\beta$ is the deactivation time fraction, and $u_0(t)$ is the excitation of the fibres in the form of a square wave.

For dynamic contractions we solve the nonlinear system of equations given by \eqref{eq:3dmuscleeqs-muscle}. For this experiment we use a block of muscle with the following dimensions: 0.52 meters long (in the x direction), 0.1375 meters wide (in the y direction), and 0.055578273 meters high (in the z direction). We attach a thin block of aponeurosis on the -z and +z faces of the muscle block with the same width and length as the muscle, and with thickness 0.0075 meters high (in the z direction). 
% Let us consider the initial configuration $V_0:=(-0.2600,0.2600)\times(-0.0688,0.0688)\times(-0.0278,0.0278)\cup(-0.2600,0.2600)\times(-0.0688,0.0688)\times(0.0278,0.0353)\cup(-0.2600,0.2600)\times(-0.0688,0.0688)\times(-0.0278,-0.0353)$.
We then shear the block in the x direction to obtain the geometry shown in \autoref{fig:3dmusclemuslewithapo} which we consider to be the initial configuration $V_0$. The -x and +x faces of the resulting geometry are given by the sets $\{\x_0\in\overline{V}_0:x_0 = -0.3364\}$ and $\{\x_0\in\overline{V}_0:x_0 = 0.3364\}$ respectively. We prescribed a Dirichlet boundary condition on $S_0:=\{\x_0\in\overline{V}_0:x_0 = -0.3364\}\cup\{\x_0\in\overline{V}_0:x_0 = 0.3364\}$. We let $V$ and $S$ be the current configuration of $V_0$ and $S_0$ respectively.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = .5\textwidth, height=.3\textheight]{muscleapo2.jpg}\includegraphics[width = .5\textwidth, height=.3\textheight]{muscleapo3.jpg}
    \centering
    \includegraphics[width = .5\textwidth, height=.3\textheight]{muscleapo1.jpg}\includegraphics[width = .5\textwidth, height=.3\textheight]{muscleapo4.jpg}
    \caption{Geometry used in this experiment. This geometry is a simplistic representation of a human medial gastrocnemius. The top right figure shows the geometry in the +x direction (yz plane). This geometry is a simplistic representation of a human medial gastrocnemius. The top left figure shows the geometry in the -x direction (yz plane). The bottom right figure displays the geometry in the $xz$ plane while the bottom left figure shows the geometry in an oblique plane.}
    \label{fig:3dmusclemuslewithapo}
\end{figure}
We specify a traction free boundary condition on $\partial V\backslash S$ at all times. The prescribed displacement on $S$ is defined as 
\begin{align*}
    \d = \begin{cases}
    \zero, & \text{on -x face, for all $t>0$},\\
    s\cdot\sin(2\pi f t)(1,0,0)^\transpose, & \text{on +x face, for all $t>0$}.
\end{cases}
\end{align*}
The parameters $s$ and $f$ represent prescribed strains and frequencies that can be specified as part of the boundary condition. The prescribed displacement on the +x face of the geometry allows to deform such face in a cyclic manner, where the displacement in the x direction is between $-s$ and $s$, and the number of cycles is determined by the frequency $f$.

The orientation of the muscle fibres is initially given as $\a_0:=(0.9397,0,0.3420)^\transpose$ while the orientation of the aponeurosis fibres is initially defined as $\a_0:= (1,0,0)^\transpose$. This gives a pennation angle of 20 degrees in the muscle fibres. A full list of the parameters used for this run is given in % \sebacomments{add full description of parameters.}
\autoref{appendix:dynamic}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = 1.0\textwidth, height=0.3\textheight]{lengthvstime.jpg}
    \includegraphics[width = 1.0\textwidth, height=0.3\textheight]{forcevstime.jpg}
    \includegraphics[width = 1.0\textwidth, height=0.3\textheight]{forcevslength.jpg}
    \caption{Muscle length (top) and force (middle) profiles in time, and work-loops (bottom) of the muscle represented by the geometry in \autoref{fig:3dmusclemuslewithapo}. 
    }
    \label{fig:3dmusclework}
\end{figure}

In \autoref{fig:3dmusclework} we plot the muscle length and force profiles in time, and the work-loop of the cyclic contraction simulated in this example. We see that muscle force increases as the activation increases. We also see a lower increase within the time intervals $[0.3,0.5]$ and $[0.8,1.0]$. We note that the increase in forces are when the activation of the muscle forces is decreasing and the muscle length is shortening below 1. This is also exhibited in the work-loop where we see that a larger loop is generated due to the combined action of both active and passive forces compared to the smaller loop generated when the normalized muscle length is shorter than 1.
Compared to the work loops obtained with one dimensional models under similar settings, we see that the relationship force-length is much more complicated in the three dimensional model from than of the one dimensional model presented in \cite{ref:ross2018-2}. The cause of the increase in force within the time intervals $[0.3,0.5]$ and $[0.8,1.0]$ may be caused by the effects of the pennation angle of the fibres, the base material, the aponeurosis, and the three dimensional architecture of the muscle. A more detailed investigation regarding the energy of muscle during dynamic contraction is subject of current research in \cite{ref:ross2020}.

% The solution to this first order ODE is
% \begin{align}
%     % a(t) := a_1(t)(H(t-t_{start})-H(t-t_{max})) + a_1(t_{max})e^{\frac{\beta}{\tau_{act}}(t_{max}-t)}(H(t-t_{max})-H(t-t_{end}))
%     a(t) := \left\{\begin{array}{rr}
%         0, & 0\leq t < t_{start}, \\
%         \frac{u_0(t)}{\beta+(1-\beta)u_0(t)}\big(1-\exp\big(
%         \frac{\beta+(1-\beta)u_0}{\tau_{act}}(t_{start}-t)\big)\big), & t_{start} \leq t < t_{max},\\
%         \frac{u_0(t)}{\beta+(1-\beta)u_0(t)}\big(1-\exp\big(
%         \frac{\beta+(1-\beta)u_0}{\tau_{act}}(t_{start}-t_{max})\big)\big)\exp\big(\frac{\beta}{\tau_{act}}(t_{max}-t)\big), & t_{max} \leq t < t_{end},
%     \end{array}\right.
% \end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Isokinetic force-velocity experiments}\label{section:3dmuscleforcevelocity}

The force-velocity relationship is a fundamental principle of skeletal muscle physiology based on Hill's studies on isolated frog muscles (\cite{Alcazaretal}). In this study, Hill found that when a muscle is stimulated isometrically and then suddenly released under a load, the shortening speed increases with decreasing loads in a hyperbolic relationship (\cite{Hill1938}). While Hill's experiments have been instrumental to our understanding of the muscle's force-velocity relationship, due to the small scale of these experiments, important factors such as mass and the 3D behaviour of muscle tissue were neglected. Due to practical and ethical considerations which hinder accurate \emph{in vivo} measures, our understanding of whole muscle behaviour remains limited. With the dynamic 3D continuum model, we can simulate isokinetic concentric contractions similar to the experiments conducted by Hill, to study the force-velocity relationship at the whole muscle level. 

Using the dynamic 3D continuum model we simulated force-velocity experiments using geometries representative of the human gastrocnemius muscle. We used a model geometry with dimensions: (length, width, height) $=  0.2080m \times 0.055m \times 0.022 m$ with a mass density of $\rho = 1060 kgm^{-3}$ to represent the approximate size of a human medial gastrocnemius muscle (\cite{Paper3}).This model was a simplified version of the human medial gastrocnemius muscle in that the muscle fibres ran parallel to the x-axis and there was no aponeurosis surrounding the muscle. The fibres had a maximum shortening rate of $5.0s^{-1}$ (normalized to resting length). To simulate an concentric (or shortening) contraction, we ran the following experiment: 
    \begin{enumerate}
        \item Lengthen the model to 1.1 of the resting length by pulling the (+x) end at a constant velocity of 1.0$s^{-1}$ (normalized by the resting length) 
        \item Five time steps of equilibrium to ensure stability. 
        \item Activate the model (uniformly) to 100\% in 0.25s using a linear ramp and fixing the (-x) and (+x) end in all directions to simulate an isometric contraction. 
        \item 15 time steps of equilibrium to increase stability.  
        \item Shorten the model to around 0.6 of the resting length by pushing on the (+x) end of the model with constant velocities (normalized by the resting length) ranging from -4.0$s^{-1}$ to -1.0$s^{-1}$
    \end{enumerate} 
For each shortening velocity, we also ran passive versions of the experiment described above where step 3 consisted of holding the (+x) and (-x) end of the model in all directions without activating it. 

Under the assumption that whole muscle acts as if individual fibres have been scaled up to the size of whole muscle (\cite{RossWakeling}), we can use Hill's force-velocity and force-length relationship to compute the theoretical force-length-velocity relationship of the whole muscle (see figure \ref{fig:intrinsic-properties-3d}). In a typical Hill-type force-velocity plot, one would plot the active force for varying shortening speeds. In the model, the total stress normal to the fibres was composed of stresses from the volumetric, active-fibres, passive-fibres, and base material (\cite{Paper1}). We defined the effective total force as the total force acting in the x-direction on the moving (+x) end in the activated model. The effective passive force was defined as the total force acting in the x-direction on the moving (+x) face in the non-activated model. The effective active force was the difference between the effective total force and the effective passive force (eq. \ref{eq:effactiveforce}). Theoretically the effective active force could equal the active force generated by the fibres, if the volumetric, passive, and base material forces are identical in the activated and passive model. Defining the effective active force in this way allows us to consider the effects of the base material when the model is activated. 
\begin{align}
	\text{effective active force} = \text{effective total force} - \text{effective passive force}
	\label{eq:effactiveforce}
\end{align}
    
\begin{figure}[!ht]  
    \noindent\makebox[\textwidth]{%
    \includegraphics[width=1.4\textwidth]{intrinsic-properties-3d.jpg}}
    \caption{Using the intrinsic stress-strain and stress-strain rate curves (see. fig. \ref{fig:intrinsic-properties-2d}, we produce force-stretch-strain rate surface plots for the total, passive, and active force. The force is normalized by the total force at optimal stretch (stretch = 1.0) and zero strain rate.}\label{fig:intrinsic-properties-3d} 
\end{figure} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}\label{section:3dmuscleconclusions}
In this paper we proposed a physical model to describe the three dimensional deformations of skeletal muscles. We used the principles of continuum mechanics to derive this model. Muscle is considered as a nearly incompressible, fibre-reinforced and transversely isotropic composite material; internal chemical reactions are triggered to produce forces which deform the tissues without any external work done on the tissues, while passive elastic properties in the muscle fibres resist the deformation in the along fibre direction. The idea of a base material was used to encapsulate the contribution from several other tissues and fluids surrounding the fibres: blood, water, extra- and intra-cellular matrix forms part of this material.  

We also proposed a numerical approach to approximate the deformations of the tissues. A semi-implicit scheme is used to discretize the time variables whereas a conforming finite element method is used to discretize the spatial variables. As a result of such time stepping, a CFL condition governs both the time step size and mesh size in order for the computation to be stable. 
Note that the implementation of our method was not optimized to match experimental data. Instead, the outputs of our model are a result of the assumptions of the physics and mechanics in our model and its implementation.

Finally, we remark that many natural processes are not considered in this study. For example, muscle contraction in living beings produces heat. Also, fluids as water and blood form part of the overall composition of muscle tissues. Even though the influence of fluids is implicitly added to our model through the experimental data we used to fit the model parameters, the current model does not explicitly consider the effects of internal fluids as part of the deformation of the tissues. Finally, chemical reactions leading to the activation of muscle fibres is not included explicitly; only the action of these reactions is encoded in our model through the active stress $\hat{\sigma}_{act}$ and the form of the activation function $a=a(t)$ as defined in \autoref{section:3dmuscledynamicexp}. These features correspond to an area of much current research which are not included in our model, and are left as future work.


==> Manuscript/dynamic.tex <==
This is a sample parameters file. The parameters shown here were used in the numerical experiment presented in \autoref{section:3dmuscledynamicexp}.
\begin{verbatim}
# Listing of Parameters
# ---------------------
subsection Finite element system
  # Displacement system polynomial order
  set Polynomial degree = 2

  # Gauss quadrature order
  set Quadrature order = 3
end

subsection Geometry
  # Global refinement level
  set Global refinement = 2

  # Global grid scaling factor
  set Grid scale = 0.1 # dimensionless

  # Length in x direction
  set Length = 0.520007951 # in m

  # Width in the y direction
  set Width = 0.1375 # in m

  # Height in the z direction
  set Height = 0.055578273 # in m

  # Curved domains
  # True if faces of geometry are transformed.
  set Curvilinear geometry = true

  # Aponeuroses thickness
  set Apo thickness = 0.0075 # in m

  # Geometry x max curvature height
  set Max x curvature height    = 0.0

  # Geometry y max curvature height
  # maximum change in height of + and - y faces due to adding curvature
  set Max y curvature height    = 0.0

  # Geometry z max curvature height
  # maximum change in height of + and - z faces due to adding curvature
  set Max z curvature height    = 0.0

  # Geometry pennation
  # Not pennation of fibres but pennation of geometry relative to global coordinate system
  set Pennation = 20.0 # relative to x axis

  # Rotate geometry w.r.t. muscle's line of action
  set Rotate LOA = true
end

subsection Import data
  # Import mesh
  set Import mesh = false # Choose whether to import an externally generated mesh

  # Mesh filename
  set Mesh filename = MTA011_mesh_with_apo_boundaries.msh # Provide the name for the mesh that you wish to import

  # Import muscle fibre activation
  set Import activation level = false # Choose whether to import an externally generated muscle fibre activation level per quadrature point

  # Muscle fibre activation filename
  set Activation level filename = fibre_activation.txt # Provide the name for the fibre activation txt file. This must be a matrix of numbers between 0 and 1, where rows represent the quadrature points and columns  represent time

  # Import fibre orientation
  set Import fibre orientation = false # Choose whether to import an externally generated fibre orientation per quadrature point

  # Fibre orientation filename
  set Fibre orientation filename = fibre_orientation.txt # Provide the name for the fibre orientation txt file. Orientation must be a unit vector

  # Import fat fraction
  set Import fat fraction = false # Choose whether to import an externally generated fat fraction per quadrature point

  # Fat fraction filename
  set Fat fraction filename = fat_fraction.txt # Provide the name for the fat fraction txt file. The fraction must be a number between 0 and 1
end


subsection Material properties
  # Type of tissue contraction
  set Contraction type = dynamic # use isometric or dynamic

  # Muscle tissue id
  # 0 : only base material
  # 1 : base material and fibre properties
  set Muscle id = 1

  # Muscle maximum isometric stress
  set Sigma naught muscle = 2.0e5 # in N/m^2 (Pa)

  # Muscle kappa value
  # Constrains how much muscle can change volume (higher = less volume change)
  set Bulk modulus muscle = 1.0e6 # in N/m^2 (Pa)

  # Maximum muscle fibre strain rate
  set Max strain rate = 5.0 # use 5.0 for slow, 10.0 for fast

  # Activation level in muscle fibres
  set Activation level = 100 # in percentage

  # Excitation level of muscle fibres
  set Excitation level = 1.0 # dimensionless values, between 0 and 1

  # Activation rate constant (tau_act in Zajac 1989)
  set Activation rate = 0.045 # dimensionless, changes with muscle fibre type

  # Deactivation rate (beta in Zajac 1989)
  set Activation beta = 0.6

  # Muscle tissue density
  set Muscle density = 1.060e+3 # in Kg/m^3

  # Muscle fibre orientation x direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle x component = 1 # dimensionless

  # Muscle fibre orientation y direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle y component = 0.0 # dimensionless

  # Muscle fibre orientation z direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle z component = 0.363970234 # dimensionless

  # Fictitious muscle base material multiplier
  # Scales muscle base material curve (higher = stiffer base material)
  set Muscle base material factor = 1.5 # dimensionless

  # Muscle base material constant 1
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 1 = 0.1990559575103343 # dimensionless

  # Muscle base material constant 2
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 2 = 0.3662334826469149 # dimensionless

  # Muscle base material constant 3
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 3 = 1.77581819784498e-8 # from fitting: 1.77581819784498e-8, dimensionless

  # Aponeurosis tissue id
  # 0 : no aponeurosis
  # 2 : aponeurosis (value of tissue id for aponeurosis)
  set Aponeurosis id = 2

  # Aponeurosis maximum isometric stress
  set Sigma naught aponeurosis = 2.0e5 # in N/m^2 (Pa)

  # Aponeurosis kappa value
  # Constrains how much the aponeurosis can change volume (higher = less volume change)
  set Bulk modulus aponeurosis = 1.0e8 # in N/m^2 (Pa)

  # Aponeurosis tissue density
  set Aponeurosis density = 1.060e+3 # in Kg/m^3

  # Aponeurosis fibre orientation x direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis x component = 1.0 # dimensionless

  # Aponeurosis fibre orientation y direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis y component = 0.0 # dimensionless

  # Aponeurosis fibre orientation z direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis z component = 0.0 # dimensionless

  # Fictitious aponeurosis base material multiplier
  # 0.1 -- Compliant Aponeurosis -- Needs to be updated! (Ryan)
  # 1.0 -- Normal Aponeurosis
  # 10.0 -- Stiff Aponeurosis -- Needs to be updated!
  set Aponeurosis base material factor = 1.0 # dimensionless

  # Aponeurosis base material constant 1
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 1 = 4.6896264975 # dimensionless

  # Aponeurosis base material constant 2
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 2 = -3.45514101975 # dimensionless

  # Aponeurosis base material constant 3
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 3 = 4.8492055395e+02 # dimensionless

  # Tendon tissue id
  # 0 : no tendon
  # 3 : tendon (currently will not work)
  set Tendon id = 0

  # Tendon maximum isometric stress
  set Sigma naught tendon = 2.0e5 # in N/m^2 (Pa)

  # Tendon kappa value
  # Constrains how much the tendon can change volume (higher = less volume change)
  set Bulk modulus tendon = 1.0e8 # in N/m^2 (Pa)

  # Tendon tissue density
  set Tendon density = 1.060e+3 # in Kg/m^3

  # Tendon fibre orientation x direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon x component = 1.0 # dimensionless

  # Tendon fibre orientation y direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon y component = 0.0 # dimensionless

  # Tendon fibre orientation z direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon z component = 0.0 # dimensionless

  # Fictitious tendon base material multiplier
  # 0.1 -- Compliant tendon -- Needs to be updated! (Ryan)
  # 1.0 -- Normal tendon
  # 10.0 -- Stiff tendon -- Needs to be updated!
  set Tendon base material factor = 1.0 # dimensionless

  # Tendon base material constant 1
  # Parameter for tendon base material curve (Yeoh 1993 model)
  set Tendon base material constant 1 = 4.6896264975 # dimensionless

  # Tendon base material constant 2
  # Parameter for tendon base material curve (Yeoh 1993 model)
  set Tendon base material constant 2 = -3.45514101975 # dimensionless

  # Tendon base material constant 3
  # Parameter for tendon base material curve (Yeoh 1993 model)
  set Tendon base material constant 3 = 4.8492055395e+02 # dimensionless

  # Fat kappa value
  # Constrains how much the fat can change volume (higher = less volume change)
  set Bulk modulus fat = 1.0e6 # in N/m^2 (Pa)

  # Fictitious fat multiplier
  # Scales the fat properties (higher = stiffer base material)
  set Fat factor = 1.0 # dimensionless

  # Fat constant 1
  # Parameter used in the fat strain energy function
  set Fat constant 1 = 0.13e6 #

  # Fat fraction within muscle
  # value should be between 0 and 1
  set Muscle fat fraction = 0.0 # 0 for fat-free muscle, 1 for fat only
end

subsection External loads
  # Strain amplitude (in the x direction)
  set Strain amplitude = 0.05 # dimensionless

  # Compression face id
  set Compression face = 6 # choose 6 for +z face or 5 for -z face

  # Compression
  # Traction applied to + z face (id 6)
  set Compression = 0.0e3 # in N/m^2 (Pa)

  # Tension face id
  set Tension face = 1 # choose 1 if no apo and 8 if adding apo

  # Given tension
  # Traction applied to + x face (id 1) if Curvilinear geometry = false
  # Traction applied to + x face of aponeurosis (id 8) if Curvilinear geometry = true
  set Tension = 0 # in N/m^2 (Pa)

  # Given volume force
  # Can use this to apply accelerations (like gravity) to the points
  set Volume force = 0.0 # in N/m^3, -1.04e+4 or -0.94e+04 for muscle (in the z direction)
end


subsection Linear solver
  # Linear solver iterations (multiples of the system matrix size)
  # In 2-d, this value is best set at 2. In 3-d, a value of 1 work fine.
  set Max iteration multiplier = 30

  # Linear solver residual (scaled by residual norm)
  set Residual                 = 1e-6

  # Use static condensation and solve a 1-block system, or solve
  # the full 3-block system using Linear Operators and the Schur
  # complement
  set Use static condensation = true

  # Solver residual
  set Residual = 1.e-6

  # Preconditioner type
  set Preconditioner type = ssor

  # Preconditioner relaxation value
  set Preconditioner relaxation  = 0.65

  # Type of solver used to solve the linear system
  set Solver type = CG # choose CG, GMRES or Direct
end


subsection Nonlinear solver
  # Type of non-linear iteration
  set non-linear solver type = classicNewton # choose classicNewton or acceleratedNewton

  # Number of Newton-Raphson iterations allowed
  set Max iterations Newton-Raphson = 4

  # Displacement error tolerance
  set Tolerance displacement = 1.0e-6 # in m

  # Force residual tolerance
  set Tolerance force = 1.0e-6 # in N
end

subsection Time
  # Type of time-stepping
  # Choose among:
  # ImpDispExpVel = explicit in the velocity, implicit in the displacement
  # FirstImpDispSemiExpVel = semi-explicit in the velocity, implicit in the displacement
  # SecondImpDispSemiExpVel = semi-explicit in the material derivative of the velocity, implicit in the displacement
  # FullyImpDisp = fully implicit in the displacement (velocity is only post-processed, not yet implemented)
  set Time stepping = ImpDispExpVel

  # Use CFL condition during computation
  set Use CFL condition = false

  # CFL condition (Cmax)
  # Not used with ImpDisp option
  set cmax = 0.05 # value should be between 0 and 1 (always positive)

  # Time step size
  set Time step size = 1.e-2 # in seconds, duration of time step

  # Tension start time
  set Tension start = 1.0 # in seconds

  # Tension end time
  set Tension end = 1.0 # in seconds

  # Compression start time
  set Compression start = 1.0 # in seconds

  # Compression end time
  set Compression end = 1.0 # in seconds

  # Activation start time
  set Activation start = 0.0 # in seconds

  # Activation end time
  set Activation end = 0.0 # in seconds

  # End time
  set End time = 1.0 # in seconds

  # For activation of fibres
  set Stim start = 0.2

  # Duty cycle
  set Duty cycle = 0.3 # dimensionless value, between 0 and 1

  # Frequency of cycles
  set Cycle frequency = 2 # in Hz
end


# 0 : No    constraint
# 1 : X     constraint
# 2 : Y     constraint
# 3 : Z     constraint
# 4 : X,Y   constraint
# 5 : X,Z   constraint
# 6 : Y,Z   constraint
# 7 : X,Y,Z constraint

subsection Boundary constraints
  # Constraints -x face tension (id 0)
  set -X constraints tension    = 0

  # Constraints +x face tension (id 1)
  set +X constraints tension    = 0

  # Constraints -y face tension (id 2)
  set -Y constraints tension    = 0

  # Constraints +y face tension (id 3)
  set +Y constraints tension    = 0

  # Constraints -z face tension (id 4)
  set -Z constraints tension    = 0

  # Constraints +z face tension (id 5)
  set +Z constraints tension    = 0

  # Constraints id 6 face tension
  set id 6 constraints tension  = 0

  # Constraints id 7 face tension
  set id 7 constraints tension  = 7

  # Constraints id 8 face tension
  set id 8 constraints tension  = 0

  #//////////////////////////////////////////////////

  # Constraints -x face compression (id 0)
  set -X constraints compression    = 7

  # Constraints +x face compression (id 1)
  set +X constraints compression    = 0

  # Constraints -y face compression (id 2)
  set -Y constraints compression    = 0

  # Constraints +y face compression (id 3)
  set +Y constraints compression    = 0

  # Constraints -z face compression (id 4)
  set -Z constraints compression    = 0

  # Constraints +z face compression (id 5)
  set +Z constraints compression    = 0

  # Constraints id 6 face compression
  set id 6 constraints compression  = 0

  # Constraints id 7 face compression
  set id 7 constraints compression  = 7

  # Constraints id 8 face compression
  set id 8 constraints compression  = 0

  #//////////////////////////////////////////////////

  # Constraints -x face active (id 0)
  set -X constraints Active   = 0

  # Constraints +x face active (id 1)
  set +X constraints Active   = 0

  # Constraints -y face active (id 2)
  set -Y constraints Active   = 0

  # Constraints +y face active (id 3)
  set +Y constraints Active   = 0

  # Constraints -z face active (id 4)
  set -Z constraints Active   = 0

  # Constraints +z face active (id 5)
  set +Z constraints Active   = 0

  # Constraints id 6 face active
  set id 6 constraints Active = 0

  # Constraints id 7 face active
  set id 7 constraints Active = 7

  # Constraints id 8 face active

  set id 8 constraints Active = 0
end
\end{verbatim}

The main C++ code was  written within the deal.ii library \cite{ref:davydov2017}, version 8.5.1. Visit \url{https://www.dealii.org/} to learn how to install and run examples on deal.ii.
% A sample code is available in the Github repository \cite{ref:dynamiccode2020}.
% \lstinputlisting[language=C++]{./Codes/dynamic-muscle.cc}


==> Manuscript/isometric.tex <==
This is a sample parameters file. The parameters shown here were used in the numerical experiment presented in \autoref{section:3dmusclecv}.
\begin{verbatim}
# Listing of Parameters
# ---------------------
subsection Finite element system
  # Displacement system polynomial order
  set Polynomial degree = 3

  # Gauss quadrature order
  set Quadrature order = 4
end

subsection Geometry
  # Global refinement level
  set Global refinement = 4

  # Global grid scaling factor
  set Grid scale = 1e-2 # dimensionless

  # Length in x direction
  set Length = 0.03 # in m

  # Width in the y direction
  set Width = 0.01 # in m

  # Height in the z direction
  set Height = 0.01 # in m

  # Curved domains
  # True if faces of geometry are transformed.
  set Curvilinear geometry = false

  # Aponeuroses thickness
  set Apo thickness = 0.00 #

  # Geometry x max curvature height
  set Max x curvature height    = 0.0

  # Geometry y max curvature height
  # maximum change in height of + and - y faces due to adding curvature
  set Max y curvature height    = 0.0

  # Geometry z max curvature height
  # maximum change in height of + and - z faces due to adding curvature
  set Max z curvature height    = 0.0

  # Geometry pennation
  # Not pennation of fibres but pennation of geometry relative to global coordinate system
  set Pennation = 0.0 # relative to x axis

  # Import mesh
  set Import mesh = false # Choose whether to import an externally generated mesh

  # Mesh filename
  set Mesh filename = mesh/block01_rot.msh # Provide the name for the mesh that you wish to import

  # Import fibre orientation
  set Import fibre orientation = false # Choose whether to import an externally generated fibre orientation per quadrature point

  # Fibre orientation filename
  set Fibre orientation filename = mesh/block01_rot_fib.txt # Provide the name for the fibre orientation txt file. Orientation must be a unit vector

  # Import fat fraction
  set Import fat fraction = false # Choose whether to import an externally generated fat fraction per quadrature point

  # Fat fraction filename
  set Fat fraction filename = mesh/ellipse_res1_fat.txt # Provide the name for the fat fraction txt file. The fraction must be a number between 0 and 1
end


subsection Material properties
  # Muscle tissue id
  # 0 : only base material
  # 1 : base material and fibre properties
  set Muscle id = 1

  # Muscle maximum isometric stress
  set Sigma naught muscle = 2.0e5 # in N/m^2 (Pa)

  # Muscle kappa value
  # Constrains how much muscle can change volume (higher = less volume change)
  set Bulk modulus muscle = 1.0e6 # in N/m^2 (Pa)

  # Activation level in muscle fibres
  set Activation level = 100 # in percentage

  # Muscle fibre orientation x direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle x component = 1.0 # dimensionless

  # Muscle fibre orientation y direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle y component = 0.0 # dimensionless

  # Muscle fibre orientation z direction
  # Determines pennation of muscle fibres relative to global coordinate system
  set Muscle z component = 0.0 # dimensionless

  # Fictitious muscle base material multiplier
  # Scales muscle base material curve (higher = stiffer base material)
  set Muscle base material factor = 1.5 # dimensionless

  # Muscle base material constant 1
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 1 = 0.1990559575103343 # dimensionless

  # Muscle base material constant 2
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 2 = 0.3662334826469149 # dimensionless

  # Muscle base material constant 3
  # Parameter for muscle base material curve (Yeoh 1993 model)
  set Muscle base material constant 3 = 1.77581819784498e-8 #  dimensionless

  # Aponeurosis tissue id
  # 0 : no aponeurosis
  # 2 : aponeurosis (value of tissue id for aponeurosis)
  set Aponeurosis id = 0

  # Aponeurosis maximum isometric stress
  set Sigma naught aponeurosis = 2.0e5 # in N/m^2 (Pa)

  # Aponeurosis kappa value
  # Constrains how much the aponeurosis can change volume (higher = less volume change)
  set Bulk modulus aponeurosis = 1.0e8 # in N/m^2 (Pa)

  # Aponeurosis fibre orientation x direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis x component = 1.0 # dimensionless

  # Aponeurosis fibre orientation y direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis y component = 0.0 # dimensionless

  # Aponeurosis fibre orientation z direction
  # Determines pennation of aponeurosis fibres relative to global coordinate system
  set Aponeurosis z component = 0.0 # dimensionless

  # Fictitious aponeurosis base material multiplier
  # 0.1 -- Compliant Aponeurosis -- Needs to be updated! (Ryan)
  # 1.0 -- Normal Aponeurosis
  # 10.0 -- Stiff Aponeurosis -- Needs to be updated!
  set Aponeurosis base material factor = 1.0 # dimensionless

  # Aponeurosis base material constant 1
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 1 = 4.6896264975 # dimensionless

  # Aponeurosis base material constant 2
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 2 = -3.45514101975 # dimensionless

  # Aponeurosis base material constant 3
  # Parameter for aponeurosis base material curve (Yeoh 1993 model)
  set Aponeurosis base material constant 3 = 4.8492055395e+02 # dimensionless

  # Tendon tissue id
  # 0 : no tendon
  # 3 : tendon (currently will not work)
  set Tendon id = 0

  # Tendon kappa value
  # Constrains how much the tendon can change volume (higher = less volume change)
  set Bulk modulus tendon = 1.0e8 # in N/m^2 (Pa)

  # Tendon fibre orientation x direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon x component = 1.0 # dimensionless

  # Tendon fibre orientation y direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon y component = 0.0 # dimensionless

  # Tendon fibre orientation z direction
  # Determines pennation of tendon fibres relative to global coordinate system
  set Tendon z component = 0.0 # dimensionless

  # Fat kappa value
  # Constrains how much the fat can change volume (higher = less volume change)
  set Bulk modulus fat = 1.0e6 # in N/m^2 (Pa)

  # Fictitious fat multiplier
  # Scales the fat properties (higher = stiffer base material)
  set Fat factor = 1.0 # dimensionless

  # Fat constant 1
  # Parameter used in the fat strain energy function
  set Fat constant 1 = 1.3e5 # 

  # Fat fraction within muscle
  # value should be between 0 and 1
  set Muscle fat fraction = 0.0 # the sum of muscle and fat fractions must add up to 1
end

subsection External loads
  # Tension face
  set Tension face = 1 # choose 1 if no apo and 8 if adding apo
  
  # Compression
  # Traction applied to + z face (id 6)
  set Compression = 0.0e3 # in N/m^2 (Pa)

  # Given tension
  # Traction applied to + x face (id 1) if Curvilinear geometry = false
  # Traction applied to + x face of aponeurosis (id 8) if Curvilinear geometry = true
  set Tension = 5e6 # in N/m^2 (Pa)

  # Given volume force
  # Can use this to apply accelerations (like gravity) to the points
  set Volume force = 0.0  # in N/m^3, -1.04e+4 or -0.94e+04 for muscle (in the z direction)
end


subsection Linear solver
  # Linear solver iterations (multiples of the system matrix size)
  # In 2-d, this value is best set at 2. In 3-d, a value of 1 work fine.
  set Max iteration multiplier = 30

  # Linear solver residual (scaled by residual norm)
  set Residual                 = 1e-6

  # Use static condensation and solve a 1-block system, or solve
  # the full 3-block system using Linear Operators and the Schur
  # complement
  set Use static condensation = true

  # Preconditioner type
  set Preconditioner type = ssor

  # Preconditioner relaxation value
  set Preconditioner relaxation  = 0.65

  # Type of solver used to solve the linear system
  set Solver type = CG # choose CG, GMRES or Direct
end


subsection Nonlinear solver
  # Type of non-linear iteration
  set non-linear solver type = classicNewton # choose classicNewton or acceleratedNewton

  # Number of Newton-Raphson iterations allowed
  set Max iterations Newton-Raphson = 5

  # Displacement error tolerance
  set Tolerance displacement = 1.0e-6 # in m

  # Force residual tolerance
  set Tolerance force = 1.0e-6 # in N
end


subsection Time
  # Time step size
    # Duration of each time step
    set Time step size = 0.05 # in seconds

    # tension start time
    set tension start = 0.0 # in seconds

    # tension end time
    set tension end = 0.5 # in seconds

    # compression start time
    set compression start = 0.0 # in seconds

    # compression end time
    set compression end = 0.0 # in seconds

    # activation start time
    set activation start = 0.5 # in seconds

    # activation end time
    set activation end = 1.0 # in seconds

    # end time
    set end time = 1.1 # in seconds
end


# 0 : No    constraint
# 1 : X     constraint
# 2 : Y     constraint
# 3 : Z     constraint
# 4 : X,Y   constraint
# 5 : X,Z   constraint
# 6 : Y,Z   constraint
# 7 : X,Y,Z constraint

subsection Boundary constraints
  # Constraints -x face tension (id 0)
  set -X constraints tension    = 7

  # Constraints +x face tension (id 1)
  set +X constraints tension    = 0

  # Constraints -y face tension (id 2)
  set -Y constraints tension    = 0

  # Constraints +y face tension (id 3)
  set +Y constraints tension    = 0

  # Constraints -z face tension (id 4)
  set -Z constraints tension    = 0

  # Constraints +z face tension (id 5)
  set +Z constraints tension    = 0

  # Constraints id 6 face tension
  set id 6 constraints tension  = 0

  # Constraints id 7 face tension
  set id 7 constraints tension  = 0

  # Constraints id 8 face tension
  set id 8 constraints tension  = 0

  #//////////////////////////////////////////////////
  
  # Constraints -x face compression (id 0)
  set -X constraints compression    = 0

  # Constraints +x face compression (id 1)
  set +X constraints compression    = 0

  # Constraints -y face compression (id 2)
  set -Y constraints compression    = 0

  # Constraints +y face compression (id 3)
  set +Y constraints compression    = 0

  # Constraints -z face compression (id 4)
  set -Z constraints compression    = 0

  # Constraints +z face compression (id 5)
  set +Z constraints compression    = 0

  # Constraints id 6 face compression
  set id 6 constraints compression  = 0

  # Constraints id 7 face compression
  set id 7 constraints compression  = 0

  # Constraints id 8 face compression
  set id 8 constraints compression  = 0
  
  #//////////////////////////////////////////////////

  # Constraints -x face active (id 0)
  set -X constraints Active   = 7

  # Constraints +x face active (id 1)
  set +X constraints Active   = 7

  # Constraints -y face active (id 2)
  set -Y constraints Active   = 0

  # Constraints +y face active (id 3)
  set +Y constraints Active   = 0

  # Constraints -z face active (id 4)
  set -Z constraints Active   = 0

  # Constraints +z face active (id 5)
  set +Z constraints Active   = 0

  # Constraints id 6 face active
  set id 6 constraints Active = 0

  # Constraints id 7 face active
  set id 7 constraints Active = 0

  # Constraints id 8 face active
  set id 8 constraints Active = 0
end
\end{verbatim}

The main C++ code was written within the deal.ii library \cite{ref:davydov2017}, version 8.5.1. Visit \url{https://www.dealii.org/} to learn how to install and run examples on deal.ii.
% A sample code is available in the Github repository \cite{ref:isometriccode2020}.
% \lstinputlisting[language=C++]{./Codes/isometric-muscle.cc}

==> Manuscript/methods.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods}\label{section:3dmusclemethods}
In this section we discribe the numerical methods and parameter fitting techniques used to simulate the three dimensional deformation of skeletal muscles.
%
% \subsection{MRI-derived geometry}
% We can utilize a realistic MRI-derived geometry with our model to solve our model for subject-specific data (\autoref{fig:MRI-mesh}), which were obtained by D'Souza et al. \cite{DSouza2019}. Using these data allows us to account for variations in the structure of muscle that may vary between subjects. This could include changes to muscle thickness, length, and volume, all of which will have an effect on the mechanics of skeletal muscle \cite{ref:lieber2000}. \autoref{fig:MRI-mesh} shows a simulation where the muscle was stretched in the $x$ direction to a whole muscle stretch of 1.1, and subsequently activated to 100\% activation at a fixed length. The $+z$ and $-z$ faces have a portion of the surface covered by an aponeurosis, which the muscle fibres insert into. The fibres in this model run at 25 degrees from the $x$ axis.
%
% \begin{figure}[!ht]
%     % \noindent\makebox[\textwidth]{%
%     \includegraphics[width=\textwidth]{Figures/MRI_MESH.pdf}}
%     \caption{Magnitude of displacement (Top) and $z$ direction displacement at 100\% activation on a subject specific MRI-derived geometry.}\label{fig:MRI-mesh}
% \end{figure}

\subsection{Determining model parameters}\label{sec:ParameterFitting}
Here we descibe the methods used to determine the parameters in the material reponse of the muscle material. The full list of parameters and function are included in the \textcolor{red}{Supplementary Material}.

\subsubsection{Volumetric response}
In this study we adopt the form of the volumetric stress used in \cite{ref:pelteret2012,ref:rahemi2014} (see also \cite{ref:holzapfel2001} for more details on volume changing free energy functions), which is typically used for nearly incompressible biological materials \cite{ref:holzapfel2001}. The volumetric part of the stress can then be defined as
\begin{align*}
    \bsigma_{vol}(J) := \frac{\kappa_{tis}}{2}\big(J-\frac{1}{J}),\,\,
    tis\in\{ecm,cell,fat,apo,ten\},
\end{align*}
in which $\kappa_{tis}>0$ is the bulk modulus of the corresponding tissue. The values for bulk moduli are determined through ensuring that the near incompressibility condition is met, ie. the values for the moduli are chosen so that there is little change in the volume of the muscle. Based on \cite{ref:blemker2005,rahemi2014regionalizing}, we choose $\kappa_{ecm} = 1\times 10^6$Pa. Due to the incompressibility of water and the fact cells are mainly composed of water we choose the volume fraction for the cellular material and fat to be $\kappa_{cell} = \kappa_{fat} = 1\times10^7 Pa$ \cite{Konno2021}. It has been shown in \cite{ref:gardiner2001,Konno2021} that the resulting strain mechanics are not very sensitive to the bulk moduli, so we mainly choose these values to ensure that the volume change is small. Due to the increased stiffness of the aponeurosis and tendon materials, the bulk modulus is chosen to be larger, $\kappa_{apo} = \kappa_{ten} = 1\times 10^8$Pa.

\subsubsection{Isochoric response}
The mechanical responses of the isochoric component of the base material for each of the different tissues uses a Yeoh model defined in terms of the Helmholtz energy as \cite{ref:yeoh1993}
\begin{align} \label{eq:YeohModel}
     \Psi_{Yeoh}(\bar\bb) := %\begin{cases}
    \sum_{k=0}^3 c_k(\tr(\bar\bb)-3)^k,\quad tis\in\{mus,apo,ten\},
\end{align}
where the constants $c_k\in\rrr$, $k=0,\ldots,3$, are determined based on experimental data.
We get the stress response, $\bsigma_{base,tiss}$, from the constituitive law
\begin{align}\label{eq:constitutiverel}
  \bsigma_{Yeoh}(\bar\bb) =2\bar\bb \frac{\partial \Psi_{Yeoh}(\bar\bb)}{\partial \bar\bb}.
\end{align}
In our model, any deformation transverse to the fibre direction will be largely due to the base material. Hence we determine the parameters, $c_k$, using experimental data for tissue pulled in the direction transverse to the fibres. Experimental data is only available for the stress as a function of stretch in a material; therefore, we use the constitutive relationship (\autoref{eq:constitutiverel}) along with the assumption of near incompressibility to express stress in terms of the principal stretch of the material. In particular, we assume that for uniaxial stretch the principal components of the stretch, $\lambda_i\in\rrr$, $i=1,\ldots,3$, are given by $\lambda = \lambda_1$ and $\lambda_2 = \lambda_3$, here $\lambda_1$ is the direction of the stretch applied in the experiment.
These relations along with $\lambda_1 \lambda_2 \lambda_3 = 1$, which comes from the incompressibility assumption, gives us the stress response from the Yeoh model as
\begin{align}
    \sigma_{Yeoh}(\lambda) = 2(\lambda^2 - \frac{1}{\lambda})\left(c_1 + 2c_2(\lambda^2 + \frac{2}{\lambda}- 3) + 3c_3(\lambda^2 + \frac{2}{\lambda} - 3)\right).
\end{align}
The parameters, $c_k$, were then obtained via non-linear regression to data from \cite{ref:mohammadkhah2016,Gillies2011decell,Alkhouli2013,Jin2013} to determine the muscle material constants and \cite{ref:mechazizi2009} for the aponeurosis and tendon base material. For the ECM component we utilize data from a decellularized ECM, which, after decellularization, undergoes material testing \cite{Gillies2011decell}. For the cellular component of the base material, obtaining mechanical data is more difficult \cite{Konno2021}. The cellular component consists largely of different cells, eg. muscle fibre cells, satellite cells, and neuron cell bodies; thus, we can utilize material data obtained from brain grey matter, which is a mass of cells with little connective tissue \cite{Jin2013}. The fat data is obtained through tensile experiments on subcutaneous fat \cite{Alkhouli2013}. This type of fat is chosen, as it has little anisotropy in the material response, which is ideal as we model the base material and therefore the fat response as isotropic. Additionally, this was the only fat data to our knowledge that contained a tensile response and was in a region near skeletal muscle, as many other studies investigated the compressive response of fat.
The parameter values from the regression are given in the \textcolor{red}{Supplementary material}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width = 0.3\textwidth]{Figures/muscle_base.pdf}
    \includegraphics[width = 0.3\textwidth]{Figures/muscle_fibre_FL.pdf}
    \includegraphics[width = 0.3\textwidth]{Figures/muscle_fibre_FV.pdf}
    \caption{Skeletal muscle material response for the isochoric component of the base material fit to data from \cite{ref:mohammadkhah2016} (A). The response for the force velocity component is fit to data from \cite{Roots2007} (B). The force-length active and passive response is fit to data from \cite{ref:winters2011} (C).}
    \label{fig:MaterialResponse}
\end{figure}

\subsubsection{Along-fibre properties}

Many different functions have been used to represent the force-length and velocity relationships \cite{Rockenfeller2017}, including trigonometric (eg. \cite{Scott1991}) and polynomial functions (eg. \cite{He1991}); however, not all these functions are equal, some will be more computationally efficient than others \cite{Rockenfeller2017}. A balanced option developed in previous work \cite{ref:ross2018-1} uses cubic Bezier curves to capture the intrinsic properties of muscle. Bezier curves are determined based on a set of polynomials that smoothly interpolate user defined points \cite{PrautzschHartmut2002BaBt}. In our case the user defined points are chosen to achieve a smooth function that accurately captures the intrinsic muscle properties. A cubic polynomial is used over higher order polynomials to allow for better local control of the function.

These Bezier curves have been used in previous 1D modelling experiments to investigate cyclic work loops \cite{ref:ross2018-1}; however, in our 3D model of muscle, they are not as practical. We opted to use a along fibre response that was twice continuously differentiable. The reason for this is that that in practice more compuational time is required to compute the resulting stress with the Bezier curve. A cubic polynomial was fit to the existing Bezier curves from \cite{ref:ross2018-1} for the passive force-length and force-velocity reponse, but with the additional requirement that the function is twice continuously differentiable everywhere. For the active force-length relationship a trigonometric function was used opposed to the polynomial fit, but with the same constraint that the function is twice continuously differentiable everywhere.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Numerical methods}

To approximate a solution of the non-linear dynamic system in \eqref{eq:3dmuscleeqs-muscle}, we use a semi-implicit time stepping for the time derivatives, and a conforming finite element scheme for the spatial variables. The displacement,
dilation, and pressure are updated with an implicit approach while the velocity is computed with an explicit update. The velocity is treated explicitly and it is only updated once the new displacement is computed.
Using this time stepping in \eqref{eq:3dmuscleeqs-muscle}, we propose
\begin{align*}
 \rho^{n}\u^{n} - \delta t^2\cdot\bdiv\,\bsigma(\u^{n},\v^{n-1},p^{n},D^{n}) =&\,\rho^{n}\u^{n-1}+\delta t\cdot\rho^{n-1}\v^{n-1} \\
 &+ \delta
t^2\cdot\big(-\bdiv(\rho^{n-1}\v^{n-1}\otimes\v^{n-1})+\b^{n}\big),\\
 D^{n} - J(\u^{n}) = 0,\quad &p^{n} - \frac{\partial\Psi_{vol}}{\partial D^{n}} = 0,\\
 \bsigma(\u^{n},\v^{n-1},p^{n},D^{n})\n = \t^{n}&,\quad \mm\u^{n} = \d^{n},
\end{align*}
where $\delta t>0$ is the timestep. The first equation comes from combining the two equations in \eqref{eq:3dmuscleeqs-muscle1} using the time discretization $\u^{n} - \delta t\v^{n} = \u^{n-1}$.

Multiplying these equations by a test function $\bchi:=(\w,q,H)\in\xx:=\hh^1(V)\times L^2(V)\times L^2(V)$ and
integrating by parts one obtains the non-linear problem: given the previous displacement $\u^{n-1}$, previous velocity $\v^{n-1}$, force $\b^{n}$,
traction $\t^{n}$, and prescribed displacement $\d^{n}$, we are to find $\bxi^{n}:=(\u^{n},p^{n},D^{n})\in\xx$ such that
\begin{align}
 a_{\v^{n-1}}(\bxi^{n},\bchi) = F_{\u^{n-1},\v^{n-1}}(\bchi),\,\,\forall\,\bchi\in\xx,\label{eq:3dmusclemuscleweakform}
\end{align}
where the map $a_{\v^{n-1}}:\xx\times\xx\to\rrr$ and the functional $F_{\u^{n-1},\v^{n-1}}:\xx\to\rrr$ are defined by
\begin{align*}
 a_{\v^{n-1}}(\bxi^{n},\bchi) &:=\, \big(\rho^{n}\u^{n},\w\big)_{V} \\
&+\delta t^2\cdot\Big\{\big(\bsigma(\u^{n},\v^{n-1},p^{n},D^{n}),\nabla\w\big)_{V}\\
&+\big(p^{n}-\frac{\partial\Psi_{vol}}{\partial D^{n}},q\big)_{V} +
\big(D^{n}-J(\u^{n}),H\big)_{V}\Big\},\\
F_{\u^{n-1},\v^{n-1}}(\bchi) &:= \,\big(\rho^{n}\u^{n-1},\w\big)_{V}+\delta t\cdot\big(\rho^{n-1}\v^{n-1},\w\big)_{V}\\&-\delta t^2\cdot\big(
\bdiv(\rho^{n-1}\v^{n-1}\otimes\v^{n-1}),\w\big)_{V}\\
&+ \delta t^2\cdot\Big\{\big(
\b^{n},\w\big)_{V} + \big(
\t^{n},\w\big)_{\partial V\backslash S}\Big\}.
\end{align*}
The non-linear nature of this problem can be handled with a Newton's iteration. We define the residual operator
$R_{\u^{n-1},\v^{n-1}}:\xx\to\xx^*$ as
\begin{align}
 [R_{\u^{n-1},\v^{n-1}}(\bxi^{n}),\bchi]_\xx := a_{\v^{n-1}}(\bxi^{n},\bchi) - F_{\u^{n-1},\v^{n-1}}(\bchi),\label{eq:3dmuscleresidual}
\end{align}
where $[\,\cdot\,,\,\cdot\,]_\xx$ denotes the duality pairing between $\xx$ and $\xx^*$.
Thus, if we assume we know a solution $\bxi^{n-1}\in\xx$ and a velocity $\v^{n-1}\in\hh^1(\Omega)$ at time step $t_n>0$, $n\in\nnn$, the Gateaux derivative for bounded functionals gives the following system: provided we have found the state $\bxi_k\in\xx$, $k\geq0$, we want to obtain a new state
$d\bxi:=(d\u,dp,dD)\in\xx$ such that
\begin{align}
 \big[\dddd R_{\v^{n-1}}(\bxi_k)(d\bxi),\bchi\big]_\xx = -\big[R_{\u^{n-1},\v^{n-1}}(\bxi_k),\bchi\big]_\xx,\quad\forall\,\bchi\in\xx.\label{eq:3dmusclelinearform}
\end{align}

To discretize the linear operator $\dddd R_{\v^{n-1}}(\bxi_k)$ in space, we utilise a standard  conforming FEM. Let $\tttt_h$ be a regular triangulation of $\overline{V}_0$ by tetrahedra $T$ of diameter $h_T$. The meshsize $h$ is defined by $h:=\max\{h_T:\,T\in\tttt_h\}$.
We use the same finite element spaces as those used in \cite{ref:pelteret2012}: the displacements are discretized with continuous polynomials whereas the pressure and dilation are discretized with discontinuous polynomials.
For a non-negative integer $k$ and
an element $T$ of $\tttt_h$, let us consider $P_k(T)$ as the space of all polynomials of degree at most $k$ defined in $T$. The space $\pp_k(T)$ would denote the vector version of $P_k(T)$. Consider the finite element spaces for $\hh^1_{\Gamma_0}(V_0)$ and $L^2(V_0)$ as
\begin{align*}
 \qq_{k+1} &:= \big\{\w\in\cc(\overline{V}_0):\,\v|_T\in\pp_{k+1}(T),\,\,\forall\,T\in\tttt_h\big\} \cap \hh^1_{\Gamma_0}(V_0),\\
 P_k &:= \big\{q\in L^2(V_0):\,q|_T\in P_k(T),\,\,\forall\,T\in\tttt_h\big\}.
\end{align*}
The discrete formulation is then as follows: given the state $\bxi_{h,k}\in\xx_h$, a previous displacement $\u^{n-1}$, and a previous velocity $\v^{n-1}$, we are to find $d\bxi_h\in\xx_h:=\qq_{k+1}\times P_k\times P_k$ such that
\begin{align}
 \big[\dddd R_{\v_h^{n-1}}(\bxi_{h,k})(d\bxi_h),\bchi_h\big] = -
\big[R_{\u_h^{n-1},\v_h^{n-1}}(\bxi_{h,k}),\bchi_h\big],\,\,\forall\,\bchi_h\in\xx_h.\label{eq:3dmusclemusclediscreteform}
\end{align}


==> Manuscript/mrigeometry.tex <==
\section{MRI-derived geometry}
We can utilize a realistic MRI-derived geometry with our model to solve our model for subject-specific data (\autoref{fig:MRI-mesh}), which were obtained by D'Souza et al. \cite{DSouza2019}. Using these data allows us to account for variations in the structure of muscle that may vary between subjects. This could include changes to muscle thickness, length, and volume, all of which will have an effect on the mechanics of skeletal muscle \cite{ref:lieber2000}. \autoref{fig:MRI-mesh} shows a simulation where the muscle was stretched in the $x$ direction to a whole muscle stretch of 1.1, and subsequently activated to 100\% activation at a fixed length. The $+z$ and $-z$ faces have a portion of the surface covered by an aponeurosis, which the muscle fibres insert into. The fibres in this model run at 25 degrees from the $x$ axis.

\begin{figure}[!ht]
    % \noindent\makebox[\textwidth]{%
    \centering\includegraphics[height=0.4\textheight, width=0.7\textwidth]{Figures/MRI_MESH.pdf}
    \caption{Magnitude of displacement (Top) and $z$ direction displacement at 100\% activation on a subject specific MRI-derived geometry. Displacements shown are in units of meters.}\label{fig:MRI-mesh}
\end{figure}

In order to use our computational framework with this more realistic geometry we need the information from post-processed MRI scans to be able to define the mesh of such geometries. We also need DTI scans to be able to map the muscle fibre orientation within such a geometry; for more details see, for instance \cite{ref:wakeling2020,Bolsterlee2021}. As one can imagine, the fibre directions inside a muscle can be quite complex. Fortunately, we only need a snapshot of the geometry and the fibre orientation vectors to be used at the beginning of the simulation, as part of the initial setup of the system.
